On the validity of the spectroscopic age indicators [Y/Mg], [Y/Al], [Y/Si], [Y/Ca], and [Y/Ti] for giant stars

The abundance ratios [Y$/$Mg], [Y$/$Al], [Y$/$Si], [Y$/$Ca], and [Y$/$Ti] have been suggested as chemical clocks for solar-metallicity dwarf stars in the field as well as for giant stars in open clusters. To verify this last hypothesis, we derive these abundances ratios of 50 giant stars belonging to seven open clusters. To calculate the abundances, we analyze FEROS spectra assuming the LTE-hypothesis. We confirm that [Y$/$Mg], [Y$/$Al], [Y$/$Si], [Y$/$Ca], and [Y$/$Ti] work as chemical clocks for field dwarf stars at the local region (d $<$ 1 kpc) whereas for the field giants the [Y$/$Mg], [Y$/$Al] and [Y$/$Si] also present trends with the ages but high scattering. [Y$/$Ca] and [Y$/$Ti] do not present any correlation with ages in the field giants. In Our open clusters, the behaviour is similar, [Y$/$Mg], [Y$/$Al] and [Y$/$Si] present evident trends, whereas [Y$/$Ca] vs. Ages is a flat and [Y$/$Ti] vs. Ages is less steep. We also confirm that the chemical clocks have high scatter at the early ages. In the case of the compiled sample, the chemical clocks are similar to our results but in some situations there are important differences. Several relations between abundance ratios and ages may be obtained when dwarfs and giants are analyzed, confirming the non-universality of the spectroscopic age indicators.

==> IC4756.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
\small
\begin{longtable}{cccccccccccccccc}
\caption{List of absorption lines for IC\,4756 stars}
\label{ic4756}\\
\hline
\hline
Wavelength  & Species & $\chi$ & log g$f$ &  E12   & E14   & E28   & E38   & E42   & E44   & E52   & E101  & E109  & E125  & E164  & Juno  \\
 (\AA)      &         &   (eV) &           &(m\AA) & (m\AA)& (m\AA)&(m\AA) & (m\AA)& (m\AA)&(m\AA) & (m\AA)& (m\AA)&(m\AA) & (m\AA)&     \\     
\hline
\hline
\endfirsthead
%
\endhead
%
5711.09 $^{1}$  & 12  & 4.34 & -1.73  &  124.7  & 136.6 & 133.7 & 117   & 113.9 & 112.1 & 143.3 & 120.1 & 124.2 & 120.4 & 121.8 & 101.4 \\
6318.71 $^{2}$  & 12  & 5.11 & -1.94  &   58.4  & 67.4  & 66.9  & 53.6  & 55.5  & 57.7  & 71.8  & 57.1  & 55.3  & ---   & 61.2  & 41.3  \\
6319.24 $^{2}$  & 12  & 5.11 & -2.17  &   36.7  & 45.6  & 47.2  & 32.2  & 33.3  & 31.1  & 46.3  & 29.2  & 36.5  & ---   & 36.7  & 28.8  \\
7387.69 $^{3}$  & 12  & 5.75 & -1.25  &   70.2  & 77    & 76.7  & 74.1  & 67.4  & 67.9  & 85.9  & 72.3  & 81.7  & 73.1  & 69.3  & 72.7  \\
7691.55 $^{2}$  & 12  & 5.75 & -1     &   71.7  & ---   & ---   & ---   & ---   & ---   & ---   & ---   & ---   & ---   & ---    & 56.2  \\
8712.69 $^{4}$  & 12  & 5.93 & -1.31  &   52.7  & ---   & ---   & ---   & ---   & ---   & ---   & ---   & ---   & ---   & ---    & 52.8  \\
8717.83 $^{5}$  & 12  & 5.93 & -1.05  &   83.2  & 89.7  & 79.5  &       & 75.5  & 71.2  & 90.6  & 77.3  & 80.9  & 73.5  &  73.5  & 79.8  \\
8736.02 $^{5}$  & 12  & 5.94 & -0.63  &  114.6  & 120.6 & 120.7 & 117.2 & 105.9 & 116.2 & 124.5 & 113.8 & 115.7 & 110.3 & 111.1  & 143.6 \\
6696.02 $^{3}$  & 13  & 3.14 & -1.481 &   54.1  & 71.4  & 76.3  & 50.9  & 49.6  & 54.5  & 90.6  & 51.6  & 57.9  & 55.3  &  58.7  & 34.3  \\
6698.67 $^{6}$  & 13  & 3.14 & -1.63  &   37.3  & 54.3  & 56.2  & 36.2  & 32.8  & 36.3  & 65.2  & 33.2  & 39.2  & 38.1  &  40.2  & 20.5  \\
7835.32 $^{6}$  & 13  & 4.04 & -0.58  &   49.6  & 54.9  & 73.5  & 49.9  & 47.1  & 50    & 77.2  & 49.7  & 57.6  & 46.1  &  52.2  & 36.7  \\
7836.13 $^{6}$  & 13  & 4.02 & -0.4   &   68    & 74.2  & 81.7  & 62.2  & ---   & 65.9  & 85.5  & 61.4  & 69.2  & 64.8  &  67.1  & 54.9  \\
8772.88 $^{6}$  & 13  & 4.02 & -0.25  &   78.7  & 102.1 & 109.4 & 83.1  & 80.1  & ---   & 110.9 &  ---  & 89.6  & ---   &  90.4  & 72.7  \\
8773.91 $^{6}$  & 13  & 4.02 & -0.07  &   ---   & 114.1 & 129.6 & ---   & 95.8  & 100.2 & 129.7 & 97.2  & 111.1 & 104.4 &  ---   & 93    \\
5488.98 $^{14}$ & 14  & 5.61 & -1.69  &   34.7  & 39.5  & 33.8  & 35.4  & 35.8  & 33.8  & 35.2  & 36.6  &  36.0 &  34.6 &  34.4  & 25.3 \\
5517.54 $^{14}$ & 14  & 5.08 & -2.50  &   22.8  & 28.3  & 24.3  & 23.8  & 23.1  & 20.9  & 28.9  & 23.8  &  24.7 &  25.5 &  26.4  & 12.3 \\
5665.55 $^{14}$ & 14  & 4.92 & -1.94  &   65.3  &  ---  & 74.1  & 59.7  & 59.4  & 60.6  & 80.3  & 63.9  &  71.1 &  60.9 &  66.6  & 40.6 \\
5684.48 $^{14}$ & 14  & 4.95 & -1.55  &   ---   &  ---  &  ---  &  ---  &  ---  & 74.1  &  ---  &  ---  &  ---  &  78.7 &  ---   & 61.1 \\
5690.43 $^{14}$ & 14  & 4.93 & -1.77  &   64.3  & 68.9  & 67.1  & 63.1  &  ---  & 62.2  & 70.5  & 66.5  &  67.8 &  63.3 &  68.8  & 47.9 \\
6125.02 $^{4}$  & 14  & 5.61 & -1.46  &   47.7  & 51.2  & 51.3  & 43.9  & 43.8  & 41.6  & 58.1  & 44.9  &  47.9 &  44.0 &  46.5  & 31.5 \\
6142.48 $^{4}$  & 14  & 5.62 & -1.29  &   43.9  & 45.6  & 45.8  & 43.6  & 47.1  & 43.6  & 44.3  & 42.4  &  45.4 &  43.3 &  40.9  & 34.1 \\
6145.02 $^{4}$  & 14  & 5.62 & -1.31  &   52.9  &  ---  & 46.1  & 47.5  &  ---  & 46.7  & 48.6  & 46.9  &  49.5 &  50.6 &  46.3  & 37.5 \\
6243.82 $^{14}$ & 14  & 5.62 & -1.24  &   58.3  & 56.3  & 58.2  & 57.8  & 55.9  & 54.1  &  ---  & 50.9  &  60.0 &  56.7 &  54.6  & 42.1 \\
6244.47 $^{14}$ & 14  & 5.62 & -1.09  &   57.3  & 57.2  & 58.7  & 61.3  & 57.8  & 57.5  & 60.1  & 52.5  &  64.0 &  57.6 &  56.5  & 42.0 \\
6414.98 $^{14}$ & 14  & 5.87 & -1.03  &   58.6  &  ---  & 52.2  & 51.3  & 58.5  & 52.9  & 58.4  & 53.3  &  61.1 &  59.2 &  56.6  & 45.1 \\
6721.85 $^{14}$ & 14  & 5.86 & -1.12  &   59.0  & 62.2  & 59.4  & 60.2  & 56.0  & 57.3  & 63.6  & 59.1  &  67.8 &  60.5 &  62.3  & 42.5 \\
6741.63 $^{14}$ & 14  & 5.98 & -1.43  &   19.5  & 21.6  & 24.5  & 20.9  &  ---  &  ---  & 26.4  & 23.4  &  ---  &  25.0 &  23.7  & 14.1 \\
6848.58 $^{15}$ & 14  & 5.86 & -1.52  &   28.1  & 29.4  &  ---  &  ---  & 27.3  & 25.1  &  ---  & 28.0  &  30.9 &  25.5 &  25.9  & 16.5 \\
7003.57 $^{15}$ & 14  & 5.96 & -0.94  &   64.4  &  ---  & 56.4  & 62.3  &  ---  &  ---  & 60.2  & 60.9  &  62.3 &  63.5 &  59.9  & 57.8 \\
5260.39 $^{6}$  & 20  & 2.52 & -1.72  &   ---   &  ---  & 67.1  & 54.8	& ---  & 51.3  &  ---	& 53.0	&	---	&  49.8	&	55.7  &	29.7  \\
5512.98 $^{6}$  & 20  & 2.93 & -0.46  &  106.6  & 122.1 & 122.7 & 103.7	& 100.6	& 104.1	& 132.3	& 100.8	& 112.0	& 102.0	&  106.2  &	83.7  \\
5581.97 $^{6}$  & 20  & 2.52 & -0.560 &  124.3  & 139.4 & 140.8 & 116.5	& 117.2	& 116.0	&	---	& 116.5	& 126.9	& 116.8	&  125.3  &	92.5  \\
5590.11 $^{14}$ & 20  & 2.52 & -0.56  &  108.4  &  ---  &  ---  & 114.4	& 109.7	&  ---  &	---	& 112.0	&	---	& 111.7	&  122.3  &	89.4  \\
5867.56 $^{14}$ & 20  & 2.93 & -1.56  &   49.2  &  58.6 &  59.8	& 37.6	&  42.1	& 37.0	&  67.3	&  41.1	&  50.0	&  40.4	&  44.8	 &	22.8  \\
6161.30 $^{4}$  & 20  & 2.52 & -1.27  &  102.0  & 114.8 &  119.1	& 93.3	&  91.7	& 95.7	& 140.2	&  91.7	& 101.2	&	92.1	&  102.2 &	64.5  \\
6166.44 $^{6}$  & 20  & 2.52 & -1.14  &  100.5  & 118.4 &  113.5	& 94.2	&  95.0	& 93.9	& 133.6	&  95.5 & 103.3	&	97.0	&  100.5 &	70.5  \\
6169.04 $^{6}$  & 20  & 2.52 & -0.79  &  117.8  & 139.6 &  136.2	& 115.2	& 112.2	& 118.9	& 149.3	&  114.7 & 125.7 &  117.3	&  120.3 &	89.3  \\
6169.56 $^{13}$ & 20  & 2.53 & -0.48  &  135.1  &  ---  &  153.1	& 131.4	& 130.5	& 136.0	&  ---	&  130.3 & 140.1 &  132.2	&  136.1 &  110.0  \\
6455.60 $^{6}$  & 20  & 2.52 & -1.33  &   87.4  & 110.6 &  109.7	& 87.9	&  84.2	&  84.1	& 123.2	&  86.6	 &  96.3 &	84.5	&   90.6 &	54.6  \\
6471.66 $^{7}$  & 20  & 2.53 & -0.69  &  122.9  & 141.7 &  142.1	& 117.3	& 115.1	& 118.5 &  ---	&  118.0 & 128.6 &  119.0   &  123.2  &   89.1  \\
6493.78 $^{13}$ & 20  & 2.52 & -0.11  &  153.2  &  ---  &   ---  &  ---  & 148.3	&   ---  &  ---	&  146.9 &  ---	 &  142.3   &   ---   &  122.2  \\
6499.65 $^{6}$  & 20  & 2.52 & -0.81  &  120.2  & 139.9 &  140.8	& 115.6	& 111.0	& 113.1	 &  ---	&  120.3 & 122.6 &  113.4   &  122.9  &   87.2  \\
6572.78 $^{15}$ & 20  & 0.00 & -4.24  &   93.2  &  ---  &   ---  &  ---  &  ---	&  95.9  &  ---	&   ---  & 110.0 &	96.1	&   ---   &   29.9  \\
7326.15 $^{15}$ & 20  & 2.93 & -0.21  &  131.4  &  ---  &  148.3	&	---	&	---	&  135.8 &	---	&	---  & 144.0 &  125.6	&	---   &  108.2  \\
5159.05    & 26      & 4.28 & -0.65  &     4   & 90.7  &  86.5  & 79.8  & 86.6  &  77.4  &  --- &  79.6  &  83.5 &    83    &  83.5   & 68.6  \\
5242.49    & 26      & 3.63 & -0.97  &  115.3  & 119.4 & 123.4 & 107.8 & 107.9 & 110.4 & 140.5 & 107.1 & 114.7 & 109.8 & 110.7 & 85.9  \\
5253.03    & 26      & 2.28 & -3.79  &   60.2  & 65.4  & 67.6  & 45.9  & 52.4  & 45.9  & 88.8  & 47.1  & 52    & 41.2  & 51.1  & 17.1  \\
5288.52    & 26      & 3.69 & -1.51  &   85.6  & 102.1 & 112.1 & 82.9  & 87.8  & 79.2  & 121.4 & 82.4  & 86.4  & 84.1  & 93.5  & 58.6  \\
5321.1     & 26      & 4.43 & -1.19  &   61.4  & 70.7  & 73.5  & 59.2  & 59.3  & 57.8  & 85.2  & 59.8  & 66    & 59.1  & 61.9  & 42.1  \\
5322.04    & 26      & 2.28 & -2.84  &  100.3  & 119.8 & 121   & 91.5  & 94.5  & 97.2  & 135.5 & 95.2  & 109.4 & 98    & 101.8 & 62.1  \\
5364.87    & 26      & 4.45 & 0.23   &  129.1  & 141   & 138.4 & 128.6 & 135   & 141   & 151.8 & 132   & 130.2 & 129.6 & 140.6 & 132.9 \\
5367.46    & 26      & 4.42 & 0.439  &  137.8  & 149.5 & 143.1 & 139.9 & 144.6 & 145.1 & 158.7 & 138.1 & 138.6 & 138.8 & 146.2 & 145.1 \\
5373.7     & 26      & 4.47 & -0.71  &   80.1  & 89.8  & 84.6  & 83.3  & 79.7  & 79.1  & 100.3 & 80.3  & 83.1  & 81    & 82.2  & 62.6  \\
5389.47    & 26      & 4.42 & -0.25  &  101.5  & 113.6 & 106.5 & 98.7  & 97.3  & 96.9  & 120   & ---    & 101.5 & 103   & 101.5 & 81.9  \\
5410.91    & 26      & 4.47 & 0.4    &  132.8  & 138.6 & 137.7 & 131.5 & 125.1 & 128.1 &  ---    & 124.6 & 133.3 & 131.7 & 127.1 & 130.9 \\
5417.03    & 26      & 4.42 & -1.53  &   55.3  & 63.9  & 60.8  & 54.6  & 52.9  & 54    & 74    & 51.5  & 57.8  & 52.2  & 58    & 35.2  \\
5441.33    & 26      & 4.31 & -1.58  &   49.9  & 71.2  & 65    & 52.4  & 52.3  & 54.8  & 74.4  & 52.2  & 56.4  & 55.4  & 48.9  & 31.5  \\
5445.04    & 26      & 4.39 & 0.041  &  123.6  & 140   & 134.6 & 125.8 & 130.7 & 122.3 & 153.1 & 128.1 & 135.6 & 126.2 & 130.2 & 122.2 \\
5522.44    & 26      & 4.21 & -1.4   &   63.3  & 68.9  & 71.8  & 63.5  & 61    & 60.5  & 81.8  & 61.9  & 64.7  & 66.1  & 60.6  & 45.1  \\
5554.89    & 26      & 4.55 & -0.38  &  122.6  & 137.3 & 136.4 & 120.5 & 118.3 & 122.7 & 139.9 & 120.7 & 129.4 & 118.9 & 125.4 & 100.1 \\
5560.21    & 26      & 4.43 & -1.04  &   72.4  & 76.8  & 75.6  & 72.9  & 64.9  & 66.9  & 84.7  & 67.6  & 71.4  & 69.6  & 67.8  & 51.1  \\
5584.76    & 26      & 3.57 & -2.17  &   63    & 77.2  & 78.4  & 58.4  & 57.8  & 61.7  & 90.8  & 62.7  & 70.1  & 63.3  & 63.8  & 39.2  \\
5624.02    & 26      & 4.39 & -1.33  &   65.1  & 76.6  & 82.5  & 72.5  & 69.1  & 62.3  & 93.5  & 69    & 73.8  & 70.2  & 71.6  & 52.3  \\
5633.94    & 26      & 4.99 & -0.12  &   78.5  & 88.1  & 85.4  & 81.8  & 79.3  & 77.5  & 98.6  & 83.2  & 85.2  & 68.5  & 83.5  & 65.2  \\
5635.82    & 26      & 4.26 & -1.74  &   51.8  & 58.4  & 56.5  & 51.6  & 50.3  & 50.6  & 68.8  & 52.8  & 54.3  & 53.4  & 54.6  & 34    \\
5638.26    & 26      & 4.22 & -0.72  &  101.6  & 114.9 & 115.1 & 94.1  & 95.7  & 99.5  & 119.3 & 98.4  & 101.6 & 103.2 & 103.1 & 77.4  \\
5691.49    & 26      & 4.3  & -1.37  &   68.1  & 72.4  & 82    & 59.9  & 63.4  & 60.3  & 94.8  & 68.2  & 75.4  & ---    & 70.1  & 40.7  \\
5705.46    & 26      & 4.3  & -1.36  &   61    & 70.6  & 72.3  & 56.9  & 61.9  & 56.9  & 77.9  & 58.8  & 63.8  & 59.6  & 62.4  & 38.8  \\
5717.83    & 26      & 4.28 & -0.979 &   87.2  & 100.5 & 98    & 85    & 87.6  & 81.2  & 106   & 85.8  & 88.5  & 85.4  & 88.7  & 63.1  \\
5731.76    & 26      & 4.26 & -1.15  &   77.5  & 88.6  & 89.6  & 78.2  & 79.2  & 78.7  & 100.5 & 82.7  & 83.9  & 84    & 86.6  & 57.4  \\
5806.72    & 26      & 4.61 & -0.9   &   71.8  & 85.5  & 86.3  & 73.2  & 73.6  & 75    & 92.5  & 77.5  & 74.8  & 78    & 76.9  & 53.9  \\
5814.8     & 26      & 4.28 & -1.82  &   39.3  & 48.5  & 51.7  & 40    & 38.3  & 39    & 58.6  & 39.3  & 46.2  & 38.8  & 40.1  & 23.4  \\
5852.21    & 26      & 4.55 & -1.18  &   59.7  & 84.1  & 84.7  & 65.4  & 54.2  & 63.8  & ---   & 63    & 72.3  & 64.5  & 64.4  & 39.9  \\
5883.81    & 26      & 3.96 & -1.21  &   86.1  & 100.6 & 97.6  & 92.6  & 84.5  & 90.7  & 111.8 & 88.4  & 92.7  & 92.3  & 90.8  & 70.5  \\
5916.24    & 26      & 2.45 & -2.99  &   95.3  & 113.1 & 120.9 & 94    & 85.9  & 93.2  & 139.6 & 95.3  & 103.2 & 98    & 101.3 & 53.3  \\
5934.65    & 26      & 3.93 & -1.02  &   98.5  & 114.4 & 112   & 99.9  & 97.9  & 96.6  & 134.2 & 100.4 & 106.6 &       & 103.4 & 75    \\
6024.05    & 26      & 4.55 & -0.06  &  118.2  & 133.9 & 129.6 & 125.7 & 122.4 & 130.5 & 137.5 & 123.8 & 127.7 & 117.8 & 128.1 & 110.4 \\
6027.05    & 26      & 4.08 & -1.09  &   87.2  & 95    & 93.1  & 90.5  & 88.1  & 88.6  & 110   & 89.9  & 95    & 84    & 95.6  & 62.5  \\
6056.00    & 26      & 4.73 & -0.4   &   84.9  & 91.3  & 88.8  & 86.2  & 86.4  & 91.4  & 105.1 & 89.1  & 88.2  & 92.2  & 87.5  & 71.1  \\
6079.00    & 26      & 4.65 & -0.97  &   62.2  & 71.8  & 70.7  & 63.6  & 56    & 60.8  & 77.3  & 65.5  & 64.3  & 61    & 67.8  & 47.4  \\
6093.64    & 26      & 4.61 & -1.35  &   47.6  & 57.7  & 59.4  & 48.5  & 49.6  & 49.2  & 65.9  & 47.3  & 53.8  & 48.9  & 54.6  & 30.1  \\
6096.66    & 26      & 3.98 & -1.78  &   56.3  & 72.3  & 71.5  & 59.3  & 61.3  & 61.5  & 84    & 60.8  & 63.9  & 61.8  & 62.6  & 37.2  \\
6120.24    & 26      & 0.91 & -5.95  &   27.4  & 56.7  & 61.6  & 23.7  & 24.2  & 30.7  & 78.1  & 21.7  & 31.2  & 26.6  & 21    & 5.1   \\
6151.61    & 26      & 2.18 & -3.29  &   86.3  & 113   & 114   & 86.6  & 81.2  & 84.9  & 127.6 & 84.8  & 93.3  & 89.1  & 90.9  & 49.2  \\
6157.72    & 26      & 4.08 & -1.11  &   90.8  & 118   & 112.6 & 92.6  & 90.3  & 90    & 122.8 & 92.9  & 102.4 & 93    & 103.9 & 63.5  \\
6165.36    & 26      & 4.14 & -1.47  &   65.1  & 80.3  & 79.5  & 70.1  & 63.5  & 64.8  & 90.7  & 67.9  & 71.9  & 68.3  & 72.9  & 44    \\
6170.5     & 26      & 4.8  & -0.38  &  107.1  &       &       & 107.8 & 109.4 & 105.4 & ---     & 105.2 & 120.6 &       & 120   & 82.9  \\
6173.33    & 26      & 2.22 & -2.88  &  108.5  & 135.4 & 134.1 & 106.8 & 103   & 102.5 & 153.1 & 108.7 & 118.9 & 107.3 & 115.4 & 67.7  \\
6187.99    & 26      & 3.94 & -1.57  &   76.8  & 88.6  & 89.9  & 70.1  & 68.5  & 72.4  & 101.3 & 74.6  & 77.6  & 74.4  & 77.8  & 47.7  \\
6200.31    & 26      & 2.61 & -2.44  &  108.1  & 130.8 & 132.9 & 111.8 & 103.4 & 108.9 & 150.6 & ---    & 121.6 & 109.5 & 109.6 & 71.7  \\
6322.68    & 26      & 2.59 & -2.43  &  117    & 135.9 & 134.4 & 108.4 & 111.7 & 109.6 & ---    & 113.6 & 126.3 & 116.6 & 120.3 & 78.6  \\
6380.74    & 26      & 4.19 & -1.32  &   77.3  & 99.1  & 94    & 79.6  & 73.9  & 85.1  & 109.3 & 74.6  & 81.5  & 77.2  & 78.6  & 53.8  \\
6392.53    & 26      & 2.28 & -4.03  &   55    & 63.2  & 72.1  & 40.3  & 43.2  & 43.8  & 85.7  & 45.7  & 55.9  & 41.4  & 47.1  & 18.2  \\
6419.95    & 26      & 4.73 & 0.09   &  101.6  & 117.4 & 114.6 & 101.3 & 100.2 & 105.9 & 125   & 104.1 & 108.3 & ---   & 108.8 & 87    \\
6469.19    & 26      & 4.84 & -0.62  &   85    & 102.1 & 100   & 84.2  & 80.9  & 82.8  & 104.9 & 81.9  & 90.4  & ---    & 92.1  & 58.4  \\
6518.36    & 26      & 2.83 & -2.3   &   90.6  & 111.6 & 108.8 & 84.5  & 83    & 87.3  & ---   & 86.5  & 97.3  & 89.7  & 92    & 58.1  \\
6574.22    & 26      & 0.99 & -5.02  &   81    & 108.1 & 113.2 & 76    & 72.5  & 76.1  & 135.9 & 76.3  & 87.8  & 76.3  & 85.2  & 29    \\
6591.31    & 26      & 4.59 & -2.07  &   21.8  & 29.1  & 28.7  & 22.4  & 17.7  & 21.4  & 38    & 22.7  & 22.4  & ---    & 24.5  & 10.5  \\
6593.87    & 26      & 2.44 & -2.42  &  125.7  & 160   & 158.5 & 127.5 & 126.1 & 133   & ---    & 122.9 & 142.6 & ---    & 136.8 & 87.5  \\
6597.56    & 26      & 4.8  & -0.92  &   60.3  & 67    & 70.4  & 66    & 60.3  & 65.7  & 76.6  & 64.3  & 67.5  & 64.3  & 64.4  & 42.4  \\
6608.02    & 26      & 2.28 & -4.03  &   48.4  & 75.9  & 78.6  & 44    & 45.1  & 50.2  & 94.9  & 44.6  & 57.1  & 51.9  & 54.6  & 17.1  \\
6609.11    & 26      & 2.56 & -2.69  &  113.1  & 139.9 & 140.4 & 105.7 & 107.2 & 104.5 &       & 105.1 & 116.7 & 111.3 & 116.1 & 68.2  \\
6646.93    & 26      & 2.61 & -3.99  &   37.2  & 62.5  & 60.3  & 32.1  & 33.6  & 32    & 72.5  & 30.3  & 40.3  & 28.1  & 35.1  & 8.2   \\
6653.85    & 26      & 4.14 & -2.52  &   21.1  & 29.1  & 28.6  & 18.8  & 17.5  & 19.9  & 32    & 20    & 21.1  & 16.7  & 23.7  & 10.9  \\
6699.14    & 26      & 4.59 & -2.19  &   19.8  & 25.6  & 26.6  & 13.1  & 18.6  & 17.8  & 29.8  & 16.9  & 18.9  & 14.2  & 18    & 7.5   \\
6703.56    & 26      & 2.76 & -3.16  &   73.9  & 98.3  & 90.2  & 69.2  & 69    & 72.4  & 113.7 & 71.7  & 78.9  & 71.3  & 75.4  & 37.8  \\
6704.48    & 26      & 4.22 & -2.66  &   12.1  & 22.1  & 17.7  & 12.8  & 12.3  & 15.4  & 25.7  & 10.4  & 12.3  & 10.4  & 15    & 6.1   \\
6710.31    & 26      & 1.8  & -4.88  &   57.6  & 96.5  & 91.9  & 54.4  & 56    & 55.6  & 112.8 & 57.2  & 67.9  & 52.7  & 66.6  & 15.7  \\
6713.74    & 26      & 4.79 & -1.6   &   34.4  & 46.4  & 44.6  & 35.2  & 36.5  & 38.3  & 52.9  & 32.9  & 39.6  & 33.6  & 38.7  & 21.4  \\
6739.52    & 26      & 1.56 & -4.95  &   42.1  & 68.2  & 72.2  & 42.1  & 38.4  & 42.1  & 88.9  & 39.8  & 49.9  & 35.4  & 47.9  & 11.8  \\
6750.15    & 26      & 2.42 & -2.62  &  115.1  & 146.2 & 144.9 & 108.6 & 106.6 & 116   & ---   & 111.2 & 124.4 & 117.4 & 119.5 & 76.2  \\
6752.70    & 26      & 4.64 & -1.2   &   66    & 84.1  & ---   & ---   &  ---  & 58.4  & ---   & 58.6  & 70.4  & ---    & 63.5  & 38.2  \\
6783.70    & 26      & 2.59 & -3.98  &   38.3  & 74.8  & 79    & 43.9  & 46.4  & 47.4  & 92.7  & 45.8  & 51.3  & 35.6  & 46.5  & 14.3  \\
6793.25    & 26      & 4.07 & -2.47  &   26.3  & 40.8  & 37.1  & 25.9  & 27    & 28.6  & 46    & 25.1  & 32.3  & 24.7  & 33    & 13.2  \\
6806.84    & 26      & 2.73 & -3.21  &   70.8  & 97    & 94.8  & 72.8  & 66.9  & 68.5  & 110.9 & 70.9  & 80.1  & 70.1  & 77.2  & 34    \\
6810.26    & 26      & 4.61 & -0.99  &   67.2  & 78.7  & 73.7  & 67.5  & 68.2  & 70.4  & 84.5  & 70.7  & 74.1  & 62.3  & 71.8  & 50    \\
6820.37    & 26      & 4.64 & -1.17  &   61    & 74.9  & 75.4  & 58.6  & 57.6  & 62.4  & 84.4  & 66.7  & 68.2  & 58.5  & 68.4  & 40.9  \\
6851.63    & 26      & 1.61 & -5.32  &   25.9  & 48.2  & 56.5  & 24.5  & 24.2  & 25.1  & 78.7  & 22    & 35.8  & 23.3  & 25.6  & 6.7   \\
6858.15    & 26      & 4.61 & -0.93  &   68.2  & 83    & 78.6  & 70.1  & 72.3  & 70.3  & 87.6  & 72.6  & 80.6  & 71.3  & 75.9  & 50.2  \\
7132.98    & 26      & 4.08 & -1.61  &   63.7  & 80.8  & 73.8  & 59.2  & 66.1  & 57.2  & 99.4  & 67.2  & 69.9  & 67.8  & 74.9  & 42.5  \\
6745.95    & 26      & 4.07 & -2.77  &  ---    & 20.3  & 19.6  & 14.6  & 16.4  & 14.2  &  ---  &  ---  & 16.9  & 15    & 14.8  & 8.3   \\
6436.40    & 26      & 4.19 & -2.46  &  ---    &  ---  & ---   & ---    & ---    & --- & 48.1  & ---   & ---   & ---   & ---   & 11.1  \\
6551.67    & 26      & 0.99 & -5.79  &  ---    &  ---  & ---   & ---    & ---    & --- & 99.7  & ---   & ---   & ---   & ---   & 6.1   \\
4993.34    & 26.1    & 2.81 & -3.67  &   58    & 55.2  & 54.1  & 54.8  & 54.7  & 57.7  & 60.4  & 57.6  & 58.4  & 65.5  & 62.6  & 38    \\
5132.65    & 26.1    & 2.81 & -4     &   39.6  & 40.3  & 34.2  & 41    & 38.6  & 35.4  & 48.6  & 40.3  & 42.5  & 44    & 41.4  & 23.8  \\
5197.55    & 26.1    & 3.23 & -2.25  &  110.7  & 105.8 & 106.9 & 106.6 & 106.1 & 104.7 & ---   & 107.2 & 109   & 109.3 & 113.9 & 81.9  \\
5234.61    & 26.1    & 3.22 & -2.24  &  105.1  & 105.7 & 101.8 & 103.1 & 102.1 & 105.8 & 101   & 105.1 & 105.6 & 105.1 & 106.5 & 81.9  \\
5284.09    & 26.1    & 2.89 & -3.01  &   85.8  & 79.8  & 82.8  & 83.8  & 84.8  & 82.3  & ---   & 85.9  & 91.3  & 92.8  & 87.8  & 66.7  \\
5325.55    & 26.1    & 3.22 & -3.17  &   60.5  & 57.7  & 52.3  & 59.1  & 60.1  & 56.6  & 53    & 62.4  & 63.3  & 64.2  & 60.4  & 38.7  \\
5414.04    & 26.1    & 3.22 & -3.62  &   48.4  & 36.4  & 40.8  & 44.5  & 41.3  & 39.2  & 39.5  & 41.7  & 45.9  & 42.3  & 40.8  & 25.9  \\
5425.24    & 26.1    & 3.2  & -3.21  &   61.3  & 58.2  & 54.4  & 58.5  & 59.7  & 61.5  & 59.7  & 58.5  & 63.5  & 65.2  & 60.9  & 39.6  \\
5991.36    & 26.1    & 3.15 & -3.56  &   50.4  & 50.7  & 53.2  & 53.6  & 53    & 50.3  & 46.6  & 56.1  & 58.9  & 53.1  & 58    & 29.9  \\
6084.09    & 26.1    & 3.2  & -3.8   &   42.6  & 39.4  & 39.1  & 40.6  & 39.8  & 37.7  & 35.7  & 43.2  & 41.1  & 44.5  & 42    & 22.2  \\
6149.24    & 26.1    & 3.89 & -2.72  &   50    & 44    & 45.7  & 48.1  & 53.2  & 44.4  & 48.7  & 55.9  & 55.1  & 51.3  & 51.8  & 37.7  \\
6247.54    & 26.1    & 3.89 & -2.34  &   69.3  & 61    & 57.1  & 67.2  & 75.8  & 61.4  & 57.6  & 71.6  & 75.5  & 76.8  & 75.9  & 55.9  \\
6416.92    & 26.1    & 3.89 & -2.68  &   53.7  & 53.8  & 52.6  & 55.5  & 55.6  & 52.1  & 51.1  & 57.4  & 58.6  & 58.9  & 59    & 39.6  \\
6432.68    & 26.1    & 2.89 & -3.58  &   62.9  & 64.3  & 57.2  & 59.2  & 62    & 59    & 63.2  & 61.1  & 65.7  & 67.4  & 65.8  & 43.1  \\
4607.34    & 38      & 0    & 0.283  &   79.9  & 99.1  & 102   & 76.9  & 72.9  & 78.8  & 118.8 & 79.1  & 88    & 80.2  & 85.8  & 41.0  \\
4883.68$^{7}$  & 39.1    & 1.08 & 0.07  &  100.8  & 125.3 & 130.5 & 93.6  & 95.8  & 106.8 & --- & 96.9  & 105.4 & 105.4 & 96.7  & 60.1  \\
5087.43$^{7}$  & 39.1    & 1.08 & -0.17  &   84.5  & 85.9  & 90.3  & 85    & 78.9  & 77.6  & ---   & 78.7  & 88.7  & 85.4  & 82.9  & 48.8  \\
5200.42$^{7}$  & 39.1    & 0.99 & -0.57  &   82.1  & 94.8  & 73.1  & 79.4  & 75    & ---    & 106.7 & 81.4  & 89.2  & 79.6  & 83    & 38.9  \\
5289.82$^{8}$  & 39.1    & 1.03 & -1.85  &   21.5  & 29.8  & 29.6  & 23    & 19.8  & 20.4  & 39.2  & 21.2  & 28.1  & 22    & 26    & 5.2   \\
5402.78$^{6}$  & 39.1    & 1.84 & -0.44  &   48    & 48.5  & 50.5  & 38.2  & 37    & 35.4  & 52.8  & 41.1  & 44.8  & 38.2  & 42.1  & 13    \\
5205.72$^{7}$  & 39.1    & 1.03 & -0.34  &  ---    &  ---  & ---    & ---   &  ---   & ---    & ---    & 75.9  & ---   & ---   &  ---   & 41.4  \\
6127.46$^{9}$  & 40      & 0.15 & -1.06  &   19.1  & 39.6  & 46    & 14.8  &  ---   & 16.2  & 62.9  & 15.2  & 23.5  & 14.8  & 21.4  & 3.8   \\
6134.57$^{9}$  & 40      & 0    & -1.28  &   11.1  & 32.4  & ---    & 10.2  & 9.3   & 11.7  & 58.9  & ---    & 15.7 & 10.9  & 15.4  & 2.2   \\
6143.18$^{9}$  & 40      & 0.07 & -1.1   &   13.8  & 39.8  & ---    & 18.2  & ---   & ---   & 70    & 13.8  & 22.7  & 14    & 18.7  & 3     \\
5385.13$^{10}$ & 40      & 0.52 & -0.64  &   ---   & 27.5  & 25.5  & ---    & 8.9   & 8.2   & 39.1  & ---   &  ---  &  ---  &  ---  & 1.9 \\
5303.53$^{8}$  & 57.1    & 0.32 & -1.35  &   26.7  & 39.2  & 40.8  & 24.7  & 21.2  & 39.2  & 53.1  & 23.3  & 32    & 22.7  & 32.8  & 3.6   \\
6390.48$^{7}$  & 57.1    & 0.32 & -1.41  &   23.3  & 46.7  & 49.4  & 23.7  & 20.1  & ---   & 59.2  & 25.6  & 35    & 25.8  & 23.5  & 3.9   \\
5880.63$^{11}$ & 57.1    & 0.24 & -1.83  &   ---    & 24.9  &  --- &  ---    & ---     & ---   & 35.2  & ---    & 16.1  & 12.1  & 21.2  & 1.4   \\
5187.46$^{8}$  & 58.1    & 1.21 & 0.3    &   29.5  & 44.6  & 43    & 30.1  & 25    & 28.6  & 52.6  & 25    & 36.4  & 29.8  & 36    & 7.5   \\
5274.24$^{8}$  & 58.1    & 1.28 & 0.389  &   40.4  & 49.8  & 45.2  & 35.1  & 30.7  & 29.2  & 55.9  & 30.6  & 43.7  & 37.4  & 38.9  & 9.8   \\
5472.3$^{8}$   & 58.1    & 1.25 & -0.19  &   17.7  & 26.2  & 23.1  & 10.8  & 14.5  & 20.3  & 23.4  & 10.9  & 14.9  & 13.8  & 22.7  & 2.4   \\
4628.16$^{7}$  & 58.1    & 0.52 & 0.01   &    ---   &  --- & ---    &  --- &  ---   &  ---  & 87.1  & ---  & ---    & ---   & --- &  17.7  \\
4811.34$^{8}$  & 60.1    & 0.06 & -1.015 &   53.7  & 75.9  & 75.6  & 51.2  & 43.8  & 54.7  & 85.8  & 50    & 55.7  & 50.4  & 53.9  & 9.3   \\
4959.12$^{8}$  & 60.1    & 0.06 & -0.916 &   63.8  & 90.6  & 91.9  & 73.8  & 63.3  & 67.2  & 115.4 & 78.2  & 84.5  & 75.8  & 78.5  & 32.4  \\
5130.59$^{7}$  & 60.1    & 1.3  & 0.1    &   42.2  & ---   & ---    & 37.5  & ---  & ---   & ---    & ---  & ---   & ---   & 44.5  & 12.6  \\
5234.19$^{7}$  & 60.1    & 0.55 & -0.46  &   53    & ---   & ---    & 48.6  & ---  & ---   & ---    & 38.9 & ---   & 44.4  & 56.4  & 5.6   \\
5319.81$^{7}$  & 60.1    & 0.55 & -0.35  &   61.2  & ---   & ---    & ---   & ---  & ---   & 87.9  & 56.4  & 63.8  & 55.3  & 62    & 13    \\
5740.88$^{8}$  & 60.1    & 1.16 & -0.56  &   15.8  & 27.8  & 10.5  & 11    & 9.9   & 10.5  & 32.3  & 17.2  & 18.8  & 15.2  & 15.7  & 2.4   \\
\hline
\hline
\end{longtable}
\noindent $^{1}$ \citet{R99}; $^{2}$ \citet{castro97}; $^{3}$ \citet{MR94}; $^{4}$ \citet{E93}; $^{5}$ \citet{WSM}; $^{6}$ \citet{R03}; $^{7}$ \citet{SN96}; $^{8}$ \citet{VWR}; $^{9}$ \citet{S96}; $^{10}$ \citet{A05}; $^{11}$ \citet{R04}; $^{13}$ \citet{DS91}; $^{14}$ \citet{mel14}; $^{15}$ \citet{sch15}


\normalsize


==> M67.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
\small
\begin{longtable}{cccccccc}
\caption{List of absorption lines for NGC\,2682 stars}
\label{m67}\\
\hline
\hline
Wavelength  & Species & $\chi$ & log g$f$  &  E 141  & E 151  & E 244  & Juno \\
 (\AA)      &         &   (eV) &           &   (m\AA) & (m\AA)& (m\AA) &      \\           
\hline
\hline
\endfirsthead
%
\endhead
%
5711.09       & 12         & 4.34  & -1.94  &  143.3 & 145    & 130.9  & 101.4   \\
6318.71       & 12         & 5.11  & -1.25  &  78.6  &  75.6  &  67.3  & 41.3    \\
7387.69       & 12         & 5.75  & -1.05  &  98.1  &  ---   &  87.8  & 72.7    \\
8717.83       & 12         & 5.93  & -1.63  &  103.2 &  94.1  &  93.2  & 79.8    \\
8736.02       & 12         & 5.94  & -0.63  &  141.5 & 140.7  &   ---  & 143.6   \\
8712.69       & 12         & 5.93  & -1.31  &   ---  &  76.8  &  71.1  & 52.8    \\
6319.24       & 12         & 5.11  & -2.17  &   ---  &  ---   &  41.9  & 28.8    \\
6696.02       & 13         & 3.14  & -1.48  &  79.4  &  ---   &  ---   & 34.3  \\
6698.67       & 13         & 3.14  & -1.58  &  60.8  &  62.1  &  48.9  & 20.5    \\
7835.32       & 13         & 4.04  & -0.4   &  70.9  &  70.2  &  69.7  & 36.7    \\
7836.13       & 13         & 4.02  & -0.283 &  91.8  &  84    &  75.8  & 54.9    \\
8772.88       & 13         & 4.02  & -0.25  &   ---  &  ---   &  98.8  & 72.7    \\
5488.98       & 14         & 5.61  & -1.69  &  ---   &  44.9  &  42.9  &  25.3  \\
5517.54       & 14         & 5.08  & -2.50  &  32.8  &  ---   &  27.8  &  12.3  \\
5665.55       & 14         & 4.92  & -1.94  &  73.1  &  79.5  &  67.7  &  40.6  \\
5684.48       & 14         & 4.95  & -1.55  &  ---   &  ---   &  ---   &  61.1  \\
5690.43       & 14         & 4.93  & -1.77  &  80.8  &  77.4  &  71.0  &  47.9  \\
6125.02       & 14         & 5.61  & -1.46  &  54.6  &   ---  &  47.6  &  31.5  \\
6142.48       & 14         & 5.62  & -1.29  &  ---   &   ---  &  ---   &  34.1  \\
6145.02       & 14         & 5.62  & -1.31  &  ---   &  57.9  &  ---   &  37.5  \\
6243.82       & 14         & 5.62  & -1.24  &  ---   &   ---  &  ---   &  42.1  \\
6244.47       & 14         & 5.62  & -1.09  &  65.4  &  72.4  &  62.8  &  42.0  \\
6414.98       & 14         & 5.87  & -1.03  &  ---   &   ---  &  ---   &  45.1  \\
6721.85       & 14         & 5.86  & -1.12  &  ---   &  67.9  &  55.5  &  42.5  \\
6741.63       & 14         & 5.98  & -1.43  &  ---   &   ---  &  ---   &  14.1  \\
6848.58       & 14         & 5.86  & -1.52  &  ---   &   37.5 &  ---   &  16.5  \\
7003.57       & 14         & 5.96  & -0.94  &  ---   &   75.4 &  ---   &  57.8  \\
5260.39       &	20	&	2.52	&	-1.72	&	---	   &	69.8   &	---	    &	29.7	\\
5512.98       &	20	&	2.93	&	-0.46	&	121.5  &	118.8  &	107.6	&	83.7	\\
5581.97       &	20	&	2.52	&	-0.56	&	143.3  &	132.7  &	121.8	&	92.5	\\
5590.11       &	20	&	2.52	&	-0.57	&	133.6  &	 ---   &	114.5	&	89.4	\\
5867.56       &	20	&	2.93	&	-1.57	&	 67.4  &	61.1   &	47.7	&	22.8	\\
6161.30       &	20	&	2.52	&	-1.27	&	125.1  &	117.4  &	95.1	&	64.5	\\
6166.44       &	20	&	2.52	&	-1.14	&	122.5  &	114.3  &	95.8	&	70.5	\\
6169.04       &	20	&	2.52	&	-0.80	&	143.6  &	134.2  &	117.8	&	89.3	\\
6169.56       &	20	&	2.53	&	-0.48	&	---    &	150.2  &	134.5	&	110.0	\\
6455.60       &	20	&	2.52	&	-1.34	&	111.9  &	110.4  &	92.5	&	54.6	\\
6471.66       &	20	&	2.53	&	-0.69	&	140.4  &	138.6  &	121.5	&	89.1	\\
6493.78       &	20	&	2.52	&	-0.11	&	 ---   &	 ---   &	---  	&	122.2	\\
6499.65       &	20	&	2.52	&	-0.82	&	140.5  &	138.5  &	122.5	&	87.2	\\
6572.78       &	20	&	0.00	&	-4.24	&	 ---   &	 ---   &	94.2	&	29.9	\\
7326.15       &	20	&	2.93	&	-0.21	&	 ---   &	 ---   &	---	    &	108.2	\\
5022.87       & 22  &   0.83    &   -0.43   &    ---   &    145.4  &   119.3    &    70.6   \\
5039.96       & 22  &   0.02    &   -1.13   &    ---   &     ---   &   128.0    &    71.1   \\
5064.65       & 22  &   0.05    &   -0.99   &    ---   &     ---   &   140.1    &    85.2   \\
5147.48       & 22  &   0.00    &   -2.01   &    ---   &    119.4  &    ---     &    34.8   \\
5210.39       & 22  &   0.05    &   -0.88   &    ---   &     ---   &   145.1    &    88.2   \\
5219.70       & 22  &   0.02    &   -2.29   &   121.6  &    121.7  &    86.3    &   28.2    \\
5295.77       & 22  &   1.07    &   -1.63   &    73.3  &     73.9  &    46.5    &   12.6    \\
5866.45       & 22  &   1.07    &   -0.84   &   132.8  &    130.3  &   100.4    &   48.7    \\
6091.17       & 22  &   2.27    &   -0.42   &    70.6  &     68.0  &    ---     &   14.9    \\
6126.22       & 22  &   1.07    &   -1.42   &    100.6 &     97.1  &    69.1    &   23.2    \\
6258.10       & 22  &   1.44    &   -0.35   &    130.7 &    128.9  &    96.9    &   51.0    \\
6261.10       & 22  &   1.43    &   -0.48   &    ---   &     ---   &   102.3    &   48.9    \\
5242.49       & 26         & 3.63  & -0.79  &  130.2 & 128.9 & 112.7 & 85.9    \\
5253.03       & 26         & 2.28  & -3.51  &  79.8  & 75.1  & 55.3  & 17.1    \\
5288.52       & 26         & 3.69  & -1.19  &  107.1 &  ---   & 93.2  & 58.6    \\
5321.1        & 26         & 4.43  & -1.84  &  73.9  & 76.9  & 58.7  & 42.1    \\
5322.04       & 26         & 2.28  & -2.23  &  119.5 & 120.5 & 99.3  & 62.1    \\
5364.87       & 26         & 4.45  & 0.71   &  149.5 & 144.7 & 144.1 & 132.9   \\
5373.7        & 26         & 4.47  & -0.25  &  96.2  & 88.4  & 79.8  & 62.6    \\
5389.47       & 26         & 4.42  & -0.53  &  113.9 & 116   & 102.1 & 81.9    \\
5417.03       & 26         & 4.42  & -1.58  &  66    & 67.5  & 57.7  & 35.2    \\
5441.33       & 26         & 4.31  & -1.041 &  71.4  & 66.5  & 55.3  & 31.5    \\
5445.04       & 26         & 4.39  & 0.4    &  150.8 & 146.8 & 134.1 & 122.2   \\
5522.44       & 26         & 4.21  & -1.38  &  78.7  & 78.8  & 67.8  & 45.1    \\
5554.89       & 26         & 4.55  & -0.04  &  138.9 & 138.1 & 127.9 & 100.1   \\
5560.21       & 26         & 4.43  & -1.17  &  81.8  & 78.3  & 72.6  & 51.1    \\
5584.76       & 26         & 3.57  & -2.33  &  83.2  & ---  & ---  & 39.2    \\
5624.02       & 26         & 4.39  & -1.12  &  86.4  & ---  & 81.1  & 52.3    \\
5633.94       & 26         & 4.99  & -0.74  &  95.2  & 88.1  & 88.1  & 65.2    \\
5635.82       & 26         & 4.26  & -1.72  &  65.7  & 69.5  & 59.4  & 34      \\
5638.26       & 26         & 4.22  & -0.36  &  121   & 111.5 & 104.6 & 77.4    \\
5705.46       & 26         & 4.3   & -1.979 &  76.7  & 72.5  & 58.5  & 38.8    \\
5717.83       & 26         & 4.28  & -0.15  &  106.8 & 106.9 & ---   & 63.1    \\
5731.76       & 26         & 4.26  & -1.9   &  97.3  & 92.8  & 80.6  & 57.4    \\
5806.72       & 26         & 4.61  & -0.82  &  90.9  & 87    & 78.3  & 53.9    \\
5814.8        & 26         & 4.28  & -1.21  &  58.4  & 55.2  & 45.4  & 23.4    \\
5883.81       & 26         & 3.96  & -1.99  &  115.3 & 110.5 & 98.8  & 70.5    \\
5916.24       & 26         & 2.45  & -2.02  &  121.3 & 114.7 & ---  & 53.3    \\
5934.65       & 26         & 3.93  & -1.09  &  112.5 & ---  & 100.4 & 75      \\
6027.05       & 26         & 4.08  & -1.4   &  103.4 & 102   & 86.9  & 62.5    \\
6056          & 26         & 4.73  & -0.97  &  96.8  & 98.5  & 90    & 71.1    \\
6079          & 26         & 4.65  & -0.35  &  80.8  & 77.8  & 66.1  & 47.4    \\
6093.64       & 26         & 4.61  & -1.78  &  63.6  & 64.8  & 50.8  & 30.1    \\
6096.66       & 26         & 3.98  & -1.95  &  74.4  & 73.1  & 59.4  & 37.2    \\
6120.24       & 26         & 0.91  & -5.29  &  62.9  & 59.6  & 31.6  & 5.1     \\
6151.61       & 26         & 2.18  & -3.11  &  112   & 109.6 & 89.8  & 49.2    \\
6157.72       & 26         & 4.08  & -1.47  &  113.4 & 112.5 & 85.3  & 63.5    \\
6165.36       & 26         & 4.14  & -1.88  &  81.5  & 83.5  & 70.7  & 44      \\
6173.33       & 26         & 2.22  & -2.57  &  138.4 & 133.4 & 110   & 67.7    \\
6187.99       & 26         & 3.94  & -1.44  &  90.6  & 90.5  & 75.7  & 47.7    \\
6200.31       & 26         & 2.61  & -2.32  &  132.1 & 130   & 115.6 & 71.7    \\
6380.74       & 26         & 4.19  & -1.09  &  98.2  & 95.8  & 89.1  & 53.8    \\
6419.95       & 26         & 4.73  & -0.46  &  125.2 & ---   & ---   & 87      \\
6436.4        & 26         & 4.19  & -2.02  &  39.5  & ---   & 30    & 11.1    \\
6574.22       & 26         & 0.99  & -5.92  &  112.1 & 109   & 84.1  & 29      \\
6597.56       & 26         & 4.8   & -0.03  &  75.1  & 68.6  & 64.5  & 42.4    \\
6608.02       & 26         & 2.28  & -4.52  &  78.3  & 76.5  & 54.1  & 17.1    \\
6653.85       & 26         & 4.14  & -2.16  &  31.8  & ---   & ---   & 10.9    \\
6703.56       & 26         & 2.76  & -3.6   &  104.6 & 94.4  & 70.2  & 37.8    \\
6713.74       & 26         & 4.79  & -1.95  &  47.7  & 45.6  & 40.1  & 21.4    \\
6739.52       & 26         & 1.56  & -4.21  &  67.7  & 64.4  & 46.6  & 11.8    \\
6806.84       & 26         & 2.73  & -3.99  &  100.6 & 96.4  & 74.1  & 34      \\
6810.26       & 26         & 4.61  & -0.17  &  87.1  & 78.6  & 67.8  & 50      \\
6820.37       & 26         & 4.64  & -1.93  &  84.7  & 79.3  & 63.2  & 40.9    \\
6858.15       & 26         & 4.61  & -0.67  &  87.1  & 82    & 77.3  & 50.2    \\
5691.49       & 26         & 4.3   & -1.37  &  ---   & 76.2  & 65.3  & 40.7    \\
5852.21       & 26         & 4.55  & -1.18  &  ---   & 83.6  & 69.9  & 39.9    \\
6024.05       & 26         & 4.55  & -0.06  &  ---   & 138.6 & 130.4 & 110.4   \\
6322.68       & 26         & 2.59  & -2.43  &  ---   & 132.8 & 117.4 & 78.6    \\
6518.36       & 26         & 2.83  & -2.3   &  ---   & 111.6 & ---  & 61.3    \\
6609.11       & 26         & 2.56  & -2.69  &  ---   & 137.6 & 115.6 & 68.2    \\
6699.14       & 26         & 4.59  & -2.19  &  ---   & 27.6  & ---  & 7.5     \\
6704.48       & 26         & 4.22  & -2.66  &  ---   & 22.2  & ---  & 6.1     \\
6750.15       & 26         & 2.42  & -2.62  &  ---   & 144.4 & 118.9 & 76.2    \\
6392.53       & 26         & 2.28  & -4.03  &  ---   &  ---  & 56.1  & 18.2    \\
6469.19       & 26         & 4.84  & -0.62  &  ---   &  ---  & 89.5  & 58.4    \\
6593.87       & 26         & 2.44  & -2.42  &  ---   &  ---  & 125.9 & 87.5    \\
6710.31       & 26         & 1.8   & -4.88  &  ---   &  ---  & 64.2  & 15.7    \\
6745.95       & 26         & 4.07  & -2.77  &  ---   &  ---  & 18.1  & 8.3     \\
6752.7        & 26         & 4.64  & -1.2   &  ---   &  ---  & 70.6  & 38.2    \\
6793.25       & 26         & 4.07  & -2.47  &  ---   &  ---  & 31.1  & 13.2    \\
4993.34       & 26.1       & 2.81  & -3.24  &  62.9  & 65.1  & 58.4  & 38      \\
5234.61       & 26.1       & 3.22  & -2.17  &  101.8 & 106.9 & 106.8 & 81.9    \\
5325.55       & 26.1       & 3.22  & -3.62  &  56.4  & 59.6  & 57.7  & 38.7    \\
5414.04       & 26.1       & 3.22  & -3.21  &  41.3  & 45.9  & 42.3  & 25.9    \\
5425.24       & 26.1       & 3.2   & -3.56  &  59.1  & 60.4  & 57.4  & 39.6    \\
5991.36       & 26.1       & 3.15  & -3.8   &  50.6  & ---   & 50.3  & 29.9    \\
6084.09       & 26.1       & 3.2   & -3.72  &  40.7  & 39.4  & 44.3  & 22.2    \\
6149.24       & 26.1       & 3.89  & -2.34  &  49.8  & 47.8  & 46.6  & 37.7    \\
6247.54       & 26.1       & 3.89  & -2.68  &  72.5  & 65.7  & 69.7  & 55.9    \\
6416.92       & 26.1       & 3.89  & -2.58  &  53.2  & 49.4  & 55.9  & 39.6    \\
6432.68       & 26.1       & 2.89  & -3.73  &  67.3  & 64.5  & 58.9  & 43.1    \\
5197.55       & 26.1       & 3.23  & -2.25  &  ---   & 103.3 & 106.3 & 81.9    \\
5132.65       & 26.1       & 2.81  & -4.00  &  ---   & ---  & 46.2  & 23.8    \\
4607.34       & 38         & 0     & 0.17   &  100.1 & 101.1 & 78.5  & 41      \\
5087.43       & 39.1       & 1.08  & -0.57  &  92.7  & 89.1  & 84.4  & 48.8    \\
5200.42       & 39.1       & 0.99  & -0.85  &  91.9  & ---   & 73.5  & 38.9    \\
5289.82       & 39.1       & 1.03  & -1.64  &  28.6  & 26.4  & 19.7  & 5.2     \\
5402.78       & 39.1       & 1.84  & -0.44  &  ---   & 43.4  & 33    & 13      \\
5385.13       & 40         & 0.52  & -0.28  &  27.5  & 23.2  & 14.6  & 1.9     \\
6134.57       & 40         & 0     & -1.1   &  34.1  & 31.4  & ---  & 2.2     \\
6143.18       & 40         & 0.07  & -1.35  &  40.3  & 36.5  & 20.3  & 3       \\
6127.46       & 40         & 0.15  & -1.06  &  ---   & ---   & 18.5  & 3.8     \\
5303.53       & 57.1       & 0.32  & -1.41  &  30.5  & 32    & 21.6  & 3.6     \\
6390.48       & 57.1       & 0.32  & -1.74  &  40.7  & 28.5  & 24.1  & 3.9     \\
4628.16       & 58.1       & 0.52  & -0.3   &  72.3  & 68.6  & 53.5  & 17.7    \\
5187.46       & 58.1       & 1.21  & 0.389  &  34.3  & 29.4  &  ---  & 7.5     \\
5274.24       & 58.1       & 1.28  & 0.015  &  44    & 42.4  & 28.9  & 9.8     \\
5472.3        & 58.1       & 1.25  & -0.19  &  ---   & 15.7  & ---   & 2.4     \\
4811.34       & 60.1       & 0.06  & -1.916 &  66.1  & 60.7  & 42.7  & 9.3     \\
4959.12       & 60.1       & 0.06  & -0.1   &  95.2  & 91.7  & 73.3  & 32.4    \\
5130.59       & 60.1       & 1.3   & 0.35   &  58.7  & ---   & ---   & 12.6    \\
5319.81       & 60.1       & 0.55  & -0.56  &  61.3  & ---   & 44.5  & 13      \\
5740.88       & 60.1       & 1.16  & 0      &  19.7  & 17.4  & ---   & 2.4     \\
5234.19       & 60.1       & 0.55  & -0.46  &  ---   & 43.8  & ---   & 5.6     \\
\hline 
\hline
\end{longtable} 
\normalsize
%\twocolumn

==> NGC5316.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
\small
\begin{longtable}{ccccccccc}
\caption{List of absorption lines for NGC\,5316 stars}
\label{ngc5316}\\
\hline
\hline
Wavelength  & Species & $\chi$ & log g$f$  & E31   & E35   & E45   & E72   & Juno  \\
 (\AA)      &         &   (eV) &           & (m\AA) & (m\AA)& (m\AA)&(m\AA)&      \\  
 \hline
 \hline
\endfirsthead
%
\endhead
%
5711.09    & 12      & 4.34 & -1.73  &  150   & 153.4 & 158.1 & 167.6 & 101.4 \\
6318.71    & 12      & 5.11 & -1.94  &  66.9  & 85.9  & 87.1  & 89.7  & 41.3  \\
8736.02    & 12      & 5.94 & -0.63  &  135.6 & 138.2 & ---   & 129.1 & 143.6 \\
7387.69    & 12      & 5.75 & -1.25  &  ---   & 89.1  & 87.9  & 94.1  & 72.7  \\
8717.83    & 12      & 5.93 & -1.05  &  ---   &  ---  & 86.5  & 96.3  & 79.8  \\
4730.04$^{6}$ & 12      & 4.34 & -2.39 &  ---  &  ---   &  ---  & 110.5 & 55.9  \\
6698.67    & 13      & 3.14 & -1.63  &  59.2  & 68    & 78.6  & 81.7  & 20.5  \\
7836.13    & 13      & 4.02 & -0.4   &  92.5  & 95.7  & 95.3  & 104.1 & 54.9  \\
8772.88    & 13      & 4.02 & -0.25  &  108.8 & ---   & ---   & ---   & 72.7  \\
6696.02    & 13      & 3.14 & -1.481 &        & 93.1  & ---   & ---   & 34.3  \\
5488.98    & 14      & 5.61 & -1.69  &   38.9 & 35.1  &  33.4 &  40.1 & 25.3  \\
5517.54    & 14      & 5.08 & -2.50  &   24.5 & 30.1  &  26.4 &  29.8 & 12.3  \\
5665.55    & 14      & 4.92 & -1.94  &   94.1 & ---   &  ---  &  ---  & 40.6  \\
5684.48    & 14      & 4.95 & -1.55  &   ---  & 87.8  &  83.7 &  ---  & 61.1  \\
5690.43    & 14      & 4.93 & -1.77  &   81.1 & 79.7  &  70.2 &  82.9 & 47.9  \\
6125.02    & 14      & 5.61 & -1.46  &   51.0 & 58.1  &  53.2 &  ---  & 31.5  \\
6142.48    & 14      & 5.62 & -1.29  &   50.9 & 44.5  &  40.1 &  ---  & 34.1  \\
6145.02    & 14      & 5.62 & -1.31  &   66.0 & 61.6  &  49.1 &  54.4 & 37.5  \\
6243.82    & 14      & 5.62 & -1.24  &   79.7 & 53.1  &  ---  &  58.1 & 42.1  \\
6244.47    & 14      & 5.62 & -1.09  &   72.1 & 55.2  &  ---  &  63.1 & 42.0  \\
6414.98    & 14      & 5.87 & -1.03  &   58.3 & 54.2  &  ---  &  ---  & 45.1  \\
6721.85    & 14      & 5.86 & -1.12  &   ---  & ---   &  60.9 &  ---  & 42.5  \\
6741.63    & 14      & 5.98 & -1.43  &   ---  & ---   &  18.3 &  ---  & 14.1  \\
6848.58    & 14      & 5.86 & -1.52  &   32.2 & ---   &  30.2 &  ---  & 16.5  \\
7003.57    & 14      & 5.96 & -0.94  &   ---  &  60.4 &  55.5 &  59.6 & 57.8  \\
5260.39    & 20	&	2.52	& -1.72	&	65.0  &	 76.7 &	 ---  &	---    	&	29.7	\\
5512.98    & 20	&	2.93	& -0.46	&	124.1 &	132.4 &	 ---  &	142.9	&	83.7	\\
5581.97    & 20	&	2.52	& -0.56	&	---   &	151.6 &	 ---  &	---    	&	92.5	\\
5590.11    & 20	&	2.52	& -0.57	&	---   &	---   &	 ---  &	---    	&	89.4	\\
5867.56    & 20	&	2.93	& -1.57	&	---   &	66.9  &	 73.3 &	68.6	&	22.8	\\
6161.30    & 20	&	2.52	& -1.27	&	131.9 &	135.5 &	137.3 &	136.8	&	64.5	\\
6166.44    & 20	&	2.52	& -1.14	&	124.4 &	127.1 &	137.5 &	143.4	&	70.5	\\
6169.04    & 20	&	2.52	& -0.80	&	149.4 &	145.0 &	 ---  &	---    	&	89.3	\\
6169.56    & 20	&	2.53	& -0.48	&	---   &	---   &	 ---  &	---    	&	110.0	\\
6455.60    & 20	&	2.52	& -1.34	&	120.1 &	129.1 &	126.7 &	130.3	&	54.6	\\
6471.66    & 20	&	2.53	& -0.69	&	---   &	---   &	 ---  &	---    	&	89.1	\\
6493.78    & 20	&	2.52	& -0.11	&	---   &	---   &	 ---  &	---    	&	122.2	\\
6499.65    & 20	&	2.52	& -0.82	&	---   &	151.9 &	 ---  &	---    	&	87.2	\\
6572.78    & 20	&	0.00	& -4.24	&	142.5 &	---   &	 ---  &	---    	&	29.9	\\
7326.15    & 20	&	2.93	& -0.21	&	---   &	---   &	 ---  &	---    	&	108.2   \\
5022.87    & 22 &   0.83    & -0.43 &   ---   & ---   &  ---  & ---     &    70.6   \\
5039.96    & 22 &   0.02    & -1.13 &   ---   & ---   &  ---  & ---     &    71.1  \\
5064.65    & 22	&	0.05	& -0.99 &	---	  &	 ---  &  ---  &	 ---	&	85.2	\\
5113.45	&	22	&	1.44	& -0.78 &   82.5  &	102.1 &	117.5 &	127.1	&	24.4	\\
5147.48	&	22	&	0.00	& -2.01 &	 ---  &	 ---  &	 ---  &	 ---	&	34.8	\\
5210.39	&	22	&	0.05	& -0.88 &	 ---  &	 ---  &	 ---  &	 ---	&	88.2	\\
5219.70	&	22	&	0.02	& -2.29 &	 ---  &	149.3 &	 ---  &	 ---	&	28.2	\\
5295.77	&	22	&	1.07	& -1.63 &	66.2  &	 86.1 &	111.3 &	 ---	&	12.6	\\
5866.45	&	22	&	1.07	& -0.84 &  151.0  &	 ---  &	 ---  &	 ---	&	48.7	\\
6091.17	&	22	&	2.27	& -0.42 &	52.7  &	 86.1 &	 92.2 &  92.2   &	14.9	\\
6126.22	&	22	&	1.07	& -1.42 &	97.2  &  ---  & 149.7 &	147.7   &   23.2	\\
6258.10	&	22	&	1.44	& -0.35 &  147.7  & 145.1 &  ---  &  ---    &   51.0	\\
6261.10	&	22	&	1.43	& -0.48 &  149.2  &	 ---  &	 ---  &	 ---    &   48.9    \\
7138.91	&	22	&	1.44	& -1.59 &   ---   &  73.3 &  91.2 &  92.2   &	6.8	\\
5253.03    & 26      & 2.28 & -3.79  &  87.5  & 86.1  & 109.3 & 106.2 & 17.1  \\
5321.1     & 26      & 4.43 & -1.19  &  94.3  & ---   & 90.4  & 93.2  & 42.1  \\
5373.7     & 26      & 4.47 & -0.71  &  122.2 & 105.2 & 112   & 119.1 & 62.6  \\
5389.47    & 26      & 4.42 & -0.25  &  142.6 &  ---  & 134.2 & 136.2 & 81.9  \\
5417.03    & 26      & 4.42 & -1.53  &  82.3  & 78.1  & 88.8  & 86.8  & 35.2  \\
5441.33    & 26      & 4.31 & -1.58  &  83.6  & 83.3  & 89.2  & 86.5  & 31.5  \\
5522.44    & 26      & 4.21 & -1.4   &  104.7 & 90.1  & 104.3 & 99.6  & 45.1  \\
5560.21    & 26      & 4.43 & -1.04  &  93.4  & 89.2  & 100.3 & 99.6  & 51.1  \\
5584.76    & 26      & 3.57 & -2.17  &  94.9  & ---  & 107.8 & 109.8 & 39.2  \\
5624.02    & 26      & 4.39 & -1.33  &  103.1 & 104.9 & 103.5 & 109.1 & 52.3  \\
5633.94    & 26      & 4.99 & -0.12  &  117.3 & 103.7 & 98.9  & 106.3 & 65.2  \\
5635.82    & 26      & 4.26 & -1.74  &  74.6  &  ---  & 85.4  & 88.9  & 34    \\
5638.26    & 26      & 4.22 & -0.72  &  134.9 & 126.6 & 135.1 & 142   & 77.4  \\
5691.49    & 26      & 4.3  & -1.37  &  114.1 & ---   & 101.2 & 103.8 & 40.7  \\
5705.46    & 26      & 4.3  & -1.36  &  94.7  & 83    & 92.6  & 93.6  & 38.8  \\
5731.76    & 26      & 4.26 & -1.15  &  113.6 & 106.8 & 121.5 & 114.3 & 57.4  \\
5806.72    & 26      & 4.61 & -0.9   &  113.9 & 104.1 & 110   & 104.9 & 53.9  \\
5814.8     & 26      & 4.28 & -1.82  &  63.9  & 63.1  & 70.1  & 65.7  & 23.4  \\
5852.21    & 26      & 4.55 & -1.18  &  106.2 & ---   &  ---  & ---   & 39.9  \\
5883.81    & 26      & 3.96 & -1.21  &  140.9 & 129.1 & 133.1 & 133.7 & 70.5  \\
6027.05    & 26      & 4.08 & -1.09  &  131.6 & 118.1 & 126.4 & ---   & 62.5  \\
6056.00    & 26      & 4.73 & -0.4   &  130.8 & 108.3 & 114.5 & 114.9 & 71.1  \\
6079.00    & 26      & 4.65 & -0.97  &  98.5  & 84.9  & 97.6  & 99    & 47.4  \\
6093.64    & 26      & 4.61 & -1.35  &  83.5  & 70.2  & 82.5  & 81.1  & 30.1  \\
6096.66    & 26      & 3.98 & -1.78  &  86.3  & 88.9  & 94.5  & 96.1  & 37.2  \\
6120.24    & 26      & 0.91 & -5.95  &  68.7  & 83.5  & 105.3 & 104   & 5.1   \\
6165.36    & 26      & 4.14 & -1.47  &  107.7 & 96.7  & 101.7 & 113.7 & 44    \\
6187.99    & 26      & 3.94 & -1.57  &  112   & 107.5 & 115.3 & 121.4 & 47.7  \\
6380.74    & 26      & 4.19 & -1.32  &  107.5 & ---   &  ---  & 124.9 & 53.8  \\
6574.22    & 26      & 0.99 & -5.02  &  149.5 & ---   &  ---  & ---   & 29    \\
6597.56    & 26      & 4.8  & -0.92  &  84.6  & 84.1  & 85.5  & 86.5  & 42.4  \\
6608.02    & 26      & 2.28 & -4.03  &  97.3  & 101.1 & 121.9 & 113.6 & 17.1  \\
6703.56    & 26      & 2.76 & -3.16  &  133.6 & 125.8 & 135.4 & 142.5 & 37.8  \\
6710.31    & 26      & 1.8  & -4.88  &  122.8 & ---   & ---   & 130   & 15.7  \\
6713.74    & 26      & 4.79 & -1.6   &  53.4  & 51.6  & 57.3  & 60.1  & 21.4  \\
6739.52    & 26      & 1.56 & -4.95  &  74    & 91.5  & 117.4 &---    & 11.8  \\
6806.84    & 26      & 2.73 & -3.21  &  121.1 & 121.6 & 135.9 & 136.1 & 34    \\
6810.26    & 26      & 4.61 & -0.99  &  105.5 & 93.6  & 106.2 & 103.5 & 50    \\
6820.37    & 26      & 4.64 & -1.17  &  87.7  & 91    & 95.6  & 95.7  & 40.9  \\
6851.63    & 26      & 1.61 & -5.32  &  73.5  & ---   & 105   & 98.4  & 6.7   \\
6858.15    & 26      & 4.61 & -0.93  &  108.3 & 92.3  & 108.2 & 99.9  & 50.2  \\
5242.49    & 26      & 3.63 & -0.97  &  ---   & 149.6 & ---   & ---   & 85.9  \\
6151.61    & 26      & 2.18 & -3.29  &  ---   & 139.9 & ---   & ---   & 49.2  \\
6518.36    & 26      & 2.83 & -2.3   &  ---   & 133.2 & ---   & ---   & 58.1  \\
6699.14    & 26      & 4.59 & -2.19  &  ---   & 28.2  & 32    & 30.3  & 7.5   \\
6704.48    & 26      & 4.22 & -2.66  &  ---   & 22.7  & 30.4  & 30    & 6.1   \\
5717.83    & 26      & 4.28 & -0.979 &  ---   & ---   & 123.2 & 130.1 & 63.1  \\
6419.95    & 26      & 4.73 & -0.09  &  ---   & ---   & 140.8 & ---   & 87    \\
6646.93    & 26      & 2.61 & -3.99  &  ---   & ---   & 83.5  & ---   & 8.2   \\
6745.95    & 26      & 4.07 & -2.77  &  ---   & ---   & 39    & ---   & 8.3   \\
7132.98    & 26      & 4.08 & -1.61  &  ---   & ---   & 112.6 & 115.3 & 42.5  \\
5132.65    & 26.1    & 2.81 & -4     &  83.8  & 56.1  & ---   & ---   & 23.8  \\
5414.04    & 26.1    & 3.22 & -3.62  &  78    & 55.2  & 56.6  & 50.2  & 25.9  \\
5425.24    & 26.1    & 3.2  & -3.21  &  101.4 & 72.8  & 69.7  & 72.3  & 39.6  \\
5991.36    & 26.1    & 3.15 & -3.56  &  86    & 67    & 52.5  & 58.7  & 29.9  \\
6084.09    & 26.1    & 3.2  & -3.8   &  80.4  & 55.7  & ---   & ---   & 22.2  \\
6149.24    & 26.1    & 3.89 & -2.72  &  100.1 & 59.6  & 55.4  & 60.1  & 37.7  \\
6247.54    & 26.1    & 3.89 & -2.34  &  126.6 & 81.2  & 75.2  & 77    & 55.9  \\
6416.92    & 26.1    & 3.89 & -2.68  &  92.8  & 68.1  & 59.9  & ---   & 39.6  \\
5234.61    & 26.1    & 3.22 & -2.24  &  ---   & 122.8 & 122.1 & 122.7 & 81.9  \\
5325.55    & 26.1    & 3.22 & -3.17  &  ---   & 72.2  & 63.9  & 67.3  & 38.7  \\
6432.68    & 26.1    & 2.89 & -3.58  &  ---   & 75.7  & 72.3  & 84.2  & 43.1  \\
4993.34    & 26.1    & 2.81 & -3.67  &  ---   & ---   & 75.8  & ---   & 38    \\
5284.09    & 26.1    & 2.89 & -3.01  &  ---   & ---   & 107.1 & ---   & 66.7  \\
5197.55    & 26.1    & 3.23 & -2.25  &  ---   & ---   & ---    & 125.3 & 81.9  \\
4607.34    & 38      & 0    & 0.283  &  134.5 & 122.4 & 143.4 & 142.7 & 41    \\
5200.42    & 39.1    & 0.99 & -0.57  &  137.8 & 111.9 & 133.6 & ---   & 38.9  \\
5289.82    & 39.1    & 1.03 & -1.85  &  54.6  & 45.5  & 52.9  & 52.3  & 5.2   \\
5402.78    & 39.1    & 1.84 & -0.44  &  86.8  & 58.4  & 59.8  & 80.4  & 13    \\
5087.43    & 39.1    & 1.08 & -0.17  &  ---   & 118.7 & ---   & ---   & 48.8  \\
5385.13    & 40      & 0.52 & -0.64  &  28.8  & 34.9  & 66.6  & 61.1  & 1.9   \\
6127.46    & 40      & 0.15 & -1.06  &  45.2  & 59.5  & ---   & ---   & 3.8   \\
6134.57    & 40      & 0    & -1.28  &  31.1  & 52.8  & 93.2  & 79.2  & 2.2   \\
6143.18    & 40      & 0.07 & -1.1   &  46.4  & 60.9  & 97.6  & 98.2  & 3     \\
5303.53    & 57.1    & 0.32 & -1.35  &  45.7  & 55.6  & 63.3  & 56.8  & 3.6   \\
6390.48    & 57.1    & 0.32 & -1.41  &  58.2  & 68.3  & 70.9  & 70.3  & 3.9   \\
5880.63    & 57.1    & 0.24 & -1.83  & ---    &  ---  & 39.5  & ---   & 1.4   \\
5187.46    & 58.1    & 1.21 & 0.3    &  61.8  & 48.8  & 68.3  & 58    & 7.5   \\
5274.24    & 58.1    & 1.28 & 0.389  &  65.2  & 55.5  & 71.5  & 67.5  & 9.8   \\
5472.3     & 58.1    & 1.25 & -0.19  &  40.8  & 21.4  & 49.3  & 25.1  & 2.4   \\
4811.34    & 60.1    & 0.06 & -1.015 &  83.6  & 96.8  & 110.9 & 95.5  & 9.3   \\
4959.12    & 60.1    & 0.06 & -0.916 &  140.1 & 135.1 & ---   & 135.9 & 32.4  \\
5740.88    & 60.1    & 1.16 & -0.56  &  32.5  & 39.1  & 44.5  & 38.3  & 2.4   \\
5234.19    & 60.1    & 0.55 & -0.46  & ---    & 82.8  & ---   & ---   & 5.6   \\
5319.81    & 60.1    & 0.55 & -0.35  & ---    &  ---  & 104.1 & ---   & 13    \\
\hline
\hline
\end{longtable}
\normalsize

==> NGC5822.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
\small
\begin{longtable}{cccccccccccccc}
\caption{List of absorption lines for NGC\,5822 stars}
\label{ngc5822}\\
\hline
\hline
Wavelength  & Species & $\chi$ & log g$f$& E6    &  E8    & E102  & E224  & E240  & E316  & E348  & E375  & E443  & Juno  \\
(\AA)       &         &   (eV) &         & (m\AA) & (m\AA)& (m\AA)&(m\AA) & (m\AA)& (m\AA)& (m\AA) &(m\AA)& (m\AA)&       \\
\hline
\hline
\endfirsthead
\endhead
5711.09    & 12      & 4.34 & -1.73   & 117.5 & 124.9 & 116.8 & 114.1 & 141.6 & 124.9 & 118.9 & 143.8 & 142.1 & 101.4 \\
6318.71    & 12      & 5.11 & -1.94   & 52.7  & 59.8  & 56.3  & 60.9  & 80    & 60.8  & 57.2  & 73.9  & 70.5  & 41.3  \\
7387.69    & 12      & 5.75 & -1.25   & 73.1  & 79.9  & 81.3  & 84.3  & 93.2  & 85.1  & 81.4  &---    & 96.8  & 72.7  \\
8717.83    & 12      & 5.93 & -1.05   & 87.7  & ---   & ---   & 88.3  & 103.2 & 103.4 & 84.5  & 110.9 & ---   & 79.8  \\
8736.02    & 12      & 5.94 & -0.63   & 125.2 & 128.1 & 139.8 & 123   & 140.8 & 148.5 & 135.3 & ---   & 147.8 & 143.6 \\
6319.24    & 12      & 5.11 & -2.17   & ---   & 45.1  & 41.8  & 40.6  & ---   & 46.9  & 44.2  & ---   & ---   & 28.8  \\
8712.69    & 12      & 5.93 & -1.31   & ---   & 58.1  & ---   & 69.7  & ---   & 65.9  & 62.6  & 84.3  & ---   & 52.8  \\
7691.55    & 12      & 5.75 & -1      & ---   & ---   & ---   &       & ---   & 89.8  & 91    & 105.2 & 100.1 & 56.2  \\
6696.02    & 13      & 3.14 & -1.481  & 52.7  & ---   & ---   & 52    & ---   & 57.7  & 57.7  & 79.4  & 76.4  & 34.3  \\
6698.67    & 13      & 3.14 & -1.63   & 40.3  & 40.2  & 29.3  & 41.6  & 70.6  & 37.4  & 36.3  & 57.3  & 56.3  & 20.5  \\
7835.32    & 13      & 4.04 & -0.58   & 59.3  & 50.5  & 52.2  & 60.3  & ---   &  ---  &  ---  & ---   & ---   & 36.7  \\
7836.13    & 13      & 4.02 & -0.4    & 69.3  & 64.7  & 66.2  & 72.7  & 96.8  & 66.6  & 65.7  & 79.8  & 82.5  & 54.9  \\
8772.88    & 13      & 4.02 & -0.25   & ---   & ---   & 79.8  & 95.5  & ---   & ---   & ---   & ---   & ---   & 72.7  \\
8773.91    & 13      & 4.02 & -0.07   & ---   & ---   & ---   & 100.5 & ---   & ---   & ---   & ---   & ---   & 93    \\
7362.30    & 13      & 4.02 & -0.748  & ---   & ---   & ---   &  ---  & ---   & 42.3  & ---   & ---   & ---   & 31.3  \\
5488.98	   & 14      & 5.61 & -1.69	  &	---   &	---   & 30.5  &	 ---  &	---   &  36.2 &	---   &	 ---  &	 ---  &	25.3  \\
5517.54    & 14      & 5.08	& -2.50   & 24.0  &	26.4  &	18.7  &  23.1 &	---   &	 ---  &	23.6  &  28.8 &  30.6 &	12.3  \\
5665.55    & 14      & 4.92	& -1.94	  &	59.5  &	64.7  &	55.6  &	 62.9 &	 ---  &	 66.4 &	65.5  &	 ---  &	 ---  &	40.6	\\
5684.48    & 14      & 4.95	& -1.55	  &	---   &	---	  &	68.5  &	 ---  &	 ---  &	 ---  &	 ---  &	 ---  &	 ---  &	61.1	\\
5690.43    & 14      & 4.93	& -1.77	  &	63.5  &	68.3  &	59.0  &	 63.8 &	 68.8 &	 67.3 &	 ---  &	 ---  &	 ---  &	47.9	\\
6125.02    & 14      & 5.61	& -1.46	  &	45.4  &	44.4  &	39.3  &	 43.5 &	 ---  &	 46.6 &	 45.4 &	 49.4 &	45.8  &	31.5	\\
6142.48    & 14      & 5.62	& -1.29	  &	44.5  &	47.8  &	40.5  &	 ---  &	 42.3 &	 47.8 &	 ---  &	 ---  &	49.2  &	34.1	\\
6145.02    & 14      & 5.62	& -1.31	  &	48.1  &	51.8  &	41.7  &	 ---  &	 ---  &	 ---  &	 ---  &	 ---  &	52.7  &	37.5	\\
6243.82    & 14      & 5.62	& -1.24	  &	51.2  &	62.3  &	50.8  &	 56.3 &	 50.1 &	 55.4 &	 59.3 &	53.4  &	57.3  &	42.1	\\
6244.47    & 14      & 5.62	& -1.09	  &	53.1  &	65.3  &	49.2  &	 57.7 &	 56.3 &	 58.1 &	 57.9 &	54.8  &	60.5  &	42.0	\\
6414.98    & 14      & 5.87	& -1.03	  &	50.0  &	---	  &	---	  &	 51.7 &	 48.6 &	 54.9 &	 ---  &	52.1  &	52.2  &	45.1	\\
6721.85    & 14      & 5.86	& -1.12	  &	58.4  &	57.9  &	54.5  &	 56.3 &	 ---  &	 61.2 &	 60.1 &	60.1  &	 ---  &	42.5	\\
6741.63    & 14      & 5.98	& -1.43	  &	22.5  &	24.2  &	20.3  &	 22.7 &	 ---  &	 ---  &	 23.4 &	21.8  &	 ---  &	14.1	\\
6848.58    & 14      & 5.86	& -1.52   &	24.9  &	26.2  &	18.3  &	 24.9 &	 ---  &	 30.2 &	 29.7 &	28.0  &	32.4  &	16.5	\\
7003.57	   & 14      & 5.96	& -0.94   &	---	  &	---	  &	59.9  &	 65.4 &	 59.6 &	 ---  &	 ---  &	60.3  &	 ---  &	57.8	\\
5260.39	   & 20      & 2.52	& -1.72	  &	53.7  &	---   &	 ---  &	 ---  &	 78.7 &	 57.1 &	 ---  &	---   &  ---  &	29.7	\\
5512.98    & 20      & 2.93	& -0.46	&	101.8 &	108.0 &	 ---  &	101.8 &	127.4 &	110.5 &	109.0 &	122.5 &	120.7	&	83.7	\\
5581.97	   & 20      & 2.52	& -0.56	&	115.8 &	122.9 &	114.3 &	116.4 &	146.3 &	122.6 &	117.7 &	136.7 &	140.3	&	92.5	\\
5590.11    & 20      & 2.52	& -0.57	&	---   &	---   &	---   &	 ---  &	133.6 &	117.6 &	---   &	133.5 &	---    	&	89.4	\\
5867.56    & 20      & 2.93	& -1.57	&	39.7  &	46.2  &	40.8  &	45.3  &	65.2  &	45.3  &	46.6  &	---   &	59.8	&	22.8	\\
6161.30    & 20      & 2.52	& -1.27	&	---   &	96.3  &	89.0  &	88.4  &	122.5 &	97.8  &	97.2  &	110.3 &	122.1	&	64.5	\\
6166.44    & 20      & 2.52	& -1.14	&	87.5  &	104.1 &	94.2  &	94.4  &	129.7 &	102.3 &	97.2  &	120.4 &	119.8	&	70.5	\\
6169.04    & 20      & 2.52	& -0.80	&	107.7 &	123.3 &	---   &	113.7 &	---   &	116.0 &	121.3 &	140.3 &	137.6	&	89.3	\\
6169.56    & 20      & 2.53	& -0.48	&	---   &	127.2 &	---   &	 ---  &	---   &	129.5 &	135.6 &	 ---  &	---    	&	110.0	\\
6455.60    & 20      & 2.52	& -1.34	&	82.3  &	87.8  &	81.7  &	86.6  &	118.1 &	88.9  &	90.3  &	115.5 &	111.7	&	54.6	\\
6471.66    & 20      & 2.53	& -0.69	&	115.5 &	120.0 &	112.4 &	120.2 &	146.8 &	120.6 &	124.7 &	147.8 &	146.4	&	89.1	\\
6493.78    & 20      & 2.52	& -0.11	&	147.8 &	145.4 &	145.5 &	 ---  &	---   &	---   &	150.0 &	 ---  &	 ---    &	122.2	\\
6499.65    & 20      & 2.52	& -0.82	&	111.7 &	122.6 &	113.2 &	116.4 &	149.4 &	121.7 &	118.1 &	144.4 &	143.5	&	87.2	\\
6572.78    & 20      & 0.00	& -4.24	&	---   &	---   &	---   &	---   &	---   &	 ---  &	 ---  &	 ---  &	 ---    &	29.9	\\
7326.15    & 20      & 2.93	& -0.21	&	---   &	---   &	---   &	---   &	---   &	 ---  &	 ---  &	 ---  &  ---    &	108.2	\\
5022.87    & 22      & 0.83	& -0.43 &	110.3 &	114.4 &	 ---  &	110.4 &  ---  &	118.7 &	116.4 &	149.7 &	 ---    &	70.6  \\
5039.96    & 22      & 0.02 & -1.13 &	117.8 &	120.5 &	115.3 &	 ---  &  ---  &	126.5 &	126.7 &	 ---  &  ---    &	71.1   \\
5064.65    & 22      & 0.05 & -0.99 &	---   &	 ---  &  ---  &	 ---  &	 ---  &	  --- &	 ---  &  ---  &  ---    &	85.2   \\
5113.45    & 22      & 1.44 & -0.78 &	57.3  &	65.6  &	 ---  &	59.5  &	109.7 &	 66.7 &	67.7  &  ---  &  93.3   &	24.4  \\
5147.48    & 22      & 0.00 & -2.01 &	85.6  &	89.2  &	 83.5 &	84.7  &	143.3 &	 ---  &	88.2  &	121.6 &	130.6	&	34.8  \\
5210.39    & 22      & 0.05 & -0.88 &	---   &	140.2 &	133.4 &	 ---  &	 ---  &	141.4 &	142.3 &	 ---  &	 ---    &	88.2      \\
5219.70    & 22      & 0.02 & -2.29 &	68.6  &	85.7  &	36.8  &	80.4  &	143.7 &	 78.7 &	85.4  &	119.8 &	121.9	&	28.2  \\
5295.77    & 22      & 1.07 & -1.63 &	41.4  &	40.2  &	 ---  &	43.2  &	 95.3 &	 42.2 &	45.3  &	 77.4 &	80.3	&	12.6  \\
5866.45    & 22      & 1.07 & -0.84 &	95.7  &	93.2  &	 ---  &	97.4  &	 ---  &	 98.9 &	98.9  &	128.2 &	138.8	&	48.7  \\
6091.17    & 22      & 2.27 & -0.42 &	32.4  &	38.6  &	37.8  &	39.5  &	 86.5 &	 46.4 &	45.2  &	 68.7 &	69.8	&	14.9  \\
6126.22    & 22      & 1.07 & -1.42 &	60.3  &	71.2  &	61.1  &	62.2  &	122.2 &	 66.4 &	67.8  &	104.2 &	103.3	&	23.2  \\
6258.10    & 22      & 1.44 & -0.35 &	89.2  &	100.3 &	90.4  &	91.5  &	147.0 &	 95.9 &	98.8  &	123.3 &	125.7	&	51.0  \\
6261.10    & 22      & 1.43 & -0.48 &	95.2  &	 ---  &	90.5  &	94.9  &	 ---  &	 94.7 &	100.3 &	127.8 &   ---   &	48.9  \\
7138.91    & 22      & 1.44 & -1.59 &	---   &	 ---  &	 ---  &	 ---  &	 ---  &   --- &  ---  &  ---  &   ---   &	6.8   \\
5242.49    & 26      & 3.63 & -0.97 &  111.1  & 112.5 & 117.7 & 109.6 & 130.7 & 114.4 & 114.3 & 127.2 & 131.3 & 85.9  \\
5253.03    & 26      & 2.28 & -3.79   & 49.3  &  ---  & 48.2  & 51.4  & 84.5  & 57.3  & 47.8  & 76.7  & 65.8  & 17.1  \\
5288.52    & 26      & 3.69 & -1.51   & 84.5  & 88.2  & 82.1  & 85.3  &       & 93.6  & 82.3  & 112.2 & 113.7 & 58.6  \\
5321.1     & 26      & 4.43 & -1.19   & 56.3  & 62.5  & 57.5  & 61.4  & 79.4  & 64.5  & 67.1  & 75.1  & 76.1  & 42.1  \\
5322.04    & 26      & 2.28 & -2.84   & 94.4  & 104.5 & 93.5  & 97.3  & 131.1 & 101.2 & 97.6  & 123.8 & 118.2 & 62.1  \\
5364.87    & 26      & 4.45 & 0.23    & 132.3 & 134.1 & 134.8 & 135.8 & ---   & 138.3 & 129.3 & 144.1 & ---   & 132.9 \\
5367.46    & 26      & 4.42 & 0.439   & 137.2 & ---   & 142.1 & 139.2 & ---   & 144.6 & 143.1 & ---   & ---   & 145.1 \\
5373.7     & 26      & 4.47 & -0.71   & 73.8  & 81.3  & 77.8  & 80.8  & 93.7  & 83.7  & 80.9  & 94.2  & 96.2  & 62.6  \\
5389.47    & 26      & 4.42 & -0.25   & 96.4  & 93.3  & 92.2  & 98.4  & 117.3 & 103.3 & 99.3  & 113.7 & 110.4 & 81.9  \\
5410.91    & 26      & 4.47 & 0.4     & 126.7 & 133.6 & 131.1 & ---   & 143.2 & 136   & 129.1 & 144.4 & ---   & 130.9 \\
5417.03    & 26      & 4.42 & -1.53   & 52.2  & 56.6  & 50.7  & 53.6  & 71.8  & 57.7  & 54.9  & 68.9  & 65.4  & 35.2  \\
5441.33    & 26      & 4.31 & -1.58   & 52.2  & 55.2  & 48.2  & 53.8  & 73.2  & 58.9  & 53.7  & 73.8  & 70.9  & 31.5  \\
5445.04    & 26      & 4.39 & 0.041   & 131.5 & 130.2 & 127.2 & 120.1 & 143.2 & 136.4 & 128   & 148.1 & 145.1 & 122.2 \\
5522.44    & 26      & 4.21 & -1.4    & 61.1  & 69.9  & 61.6  & 63.5  & 80.5  & 67.9  & 62.5  & 85    & 79.7  & 45.1  \\
5554.89    & 26      & 4.55 & -0.38   & 116.6 & ---   & 117.2 & 121.4 & 142.7 & 125.2 & 121.4 & 140.1 & 138.2 & 100.1 \\
5560.21    & 26      & 4.43 & -1.04   & 66.6  & 73.1  & 66.6  & 68.3  & 81.5  & 71.6  & 72.4  & 82.3  & 81.7  & 51.1  \\
5584.76    & 26      & 3.57 & -2.17   & 59.4  & 69.2  & 69.4  & 60.4  & ---   & 67.5  & 61.6  & 81.8  & ---   & 39.2  \\
5624.02    & 26      & 4.39 & -1.33   & 70    & 73.4  & 67.3  & 70.3  & 92.4  & 77.3  & 72.6  & 89.6  & 89.3  & 52.3  \\
5633.94    & 26      & 4.99 & -0.12   & 78.1  & 82.5  & 82.7  & 82.2  & 94.6  & 85.2  & 77.3  & 95    & 97    & 65.2  \\
5635.82    & 26      & 4.26 & -1.74   & 51    & 53.3  & 45.4  & 50.7  & 67.7  & 57    & 58.7  & 65.3  & 71.6  & 34    \\
5638.26    & 26      & 4.22 & -0.72   & 94.8  & 101.1 & 92.3  & 95.1  & 117.3 & 101.4 & 102.1 & 114.1 & 115.4 & 77.4  \\
5691.49    & 26      & 4.3  & -1.37   & 66.9  & ---   & 67.3  & 69.6  & ---   & 63.6  & 63.2  & 87.4  & 72.1  & 40.7  \\
5705.46    & 26      & 4.3  & -1.36   & 57.5  & 61.7  & 54.4  & 56.4  & 76.8  & 65.3  & 59.3  & 76.3  & 72.9  & 38.8  \\
5731.76    & 26      & 4.26 & -1.15   & 72.2  & 79.2  & 68.2  & 76.5  & 99.9  & 84.7  & 85.5  & 98.2  & 97.4  & 57.4  \\
5806.72    & 26      & 4.61 & -0.9    & 72.8  & ---   & 68.8  & 69.6  & 92.1  & 77.1  & 76.5  & 89.3  & 87.6  & 53.9  \\
5814.8     & 26      & 4.28 & -1.82   & 37.2  & 41.4  & 37.9  & 39.3  & 57    & 42.6  & 40.9  & 55.3  & 51.4  & 23.4  \\
5852.21    & 26      & 4.55 & -1.18   & 61.2  & 65.7  & 61.1  & 65.6  &---    & 68.6  & 64.3  & 86.9  & 88.5  & 39.9  \\
5883.81    & 26      & 3.96 & -1.21   & 89.6  & 90.6  & 80.2  & 87.6  & 119.3 & 94.4  & 91.3  & 106.2 & 105.5 & 70.5  \\
5934.65    & 26      & 3.93 & -1.02   & 93.4  & 101.2 & 96.4  & 96.5  & 132.3 & 104.2 & 101.3 & ---   & 117.5 & 75    \\
6024.05    & 26      & 4.55 & -0.06   & 119   & 126.3 & 112.4 & 119.7 & 134.8 & 131.7 & 117.3 & 138.3 & 135.3 & 110.4 \\
6027.05    & 26      & 4.08 & -1.09   & 83.3  & 89.4  & 81.3  & 84.5  & 106.5 & 86.3  & 85.7  & 98.5  & 104.6 & 62.5  \\
6056       & 26      & 4.73 & -0.4    & 80    & 88.6  & 78.5  & 83.2  & 96.3  & ---   & 90.4  & 101.8 & 113.8 & 71.1  \\
6079       & 26      & 4.65 & -0.97   & 59.3  & 68.1  & 62.7  & 61.3  & 77.5  & 68.1  & 67.4  & 77.1  & 77.4  & 47.4  \\
6093.64    & 26      & 4.61 & -1.35   & 46.7  & 52.6  & 45.3  & 47.6  & 64.2  & 50.5  & 49.2  & 60.6  & 61.3  & 30.1  \\
6096.66    & 26      & 3.98 & -1.78   & 56.9  & 61.8  & 50.2  & 55.1  & 79.8  & 62.4  & 58.4  & 77.4  & 78.6  & 37.2  \\
6151.61    & 26      & 2.18 & -3.29   & 84.8  & 91.6  & 80.3  & 84.3  & 125.5 & 90.9  & 86.3  & 114.3 & 114.7 & 49.2  \\
6157.72    & 26      & 4.08 & -1.11   & 90.1  & 81.4  & 78.5  & 92.6  &---    & 98.2  & 93.2  & 103.3 & 119.9 & 63.5  \\
6165.36    & 26      & 4.14 & -1.47   & 63.3  & 67.7  & 61.1  & 64.1  & 88.5  & 71.1  & 67.8  & 86.3  & 89.9  & 44    \\
6170.5     & 26      & 4.8  & -0.38   & 100.8 & ---   &  ---  & 104.3 & ---   & 109.2 & 106.1 & ---   & 106.3 & 82.9  \\
6173.33    & 26      & 2.22 & -2.88   & 104.6 & 114.3 & 101.1 & 103.2 & ---   & 112.3 & 105.4 & 140.4 & 132.4 & 67.7  \\
6187.99    & 26      & 3.94 & -1.57   & 67.4  & 75.5  & 65.6  & 70.3  & 96.5  & 79.7  & 74.6  & 94.8  & 91.6  & 47.7  \\
6200.31    & 26      & 2.61 & -2.44   & 101.3 & 114.5 & 106.3 & 106.2 & 141.5 & 114.3 & 109.4 & 133.2 & 136.7 & 71.7  \\
6322.68    & 26      & 2.59 & -2.43   & 109.6 & 117.2 & 107.9 & 112.1 & 148.2 & 121   & 110.6 & 141.1 & 139.2 & 78.6  \\
6380.74    & 26      & 4.19 & -1.32   & 78.8  & 83.3  & 72.5  & 78.2  & 105.3 & 80.2  & 72.7  & 100.6 & 96.4  & 53.8  \\
6392.53    & 26      & 2.28 & -4.03   & 42.4  & 52.2  & 41.7  & 43.3  & 84.4  & 51.5  & 48.3  & 75.3  & 72.3  & 18.2  \\
6419.95    & 26      & 4.73 & -0.09   & 100.5 & 104.1 & 96.7  & 100.6 & 121.6 & 105.3 & 102.7 & 120.6 & 119.5 & 87    \\
6469.19    & 26      & 4.84 & -0.62   & 80.4  & ---   & 85.7  & 83.5  & ---   & 86.8  & 81.9  & ---   & 102.5 & 58.4  \\
6518.36    & 26      & 2.83 & -2.3    & 86.4  & 91.1  & 91.3  & 93.3  & 129.3 & 93.1  & 90.3  & 114.2 & 114.4 & 58.1  \\
6574.22    & 26      & 0.99 & -5.02   & 75.8  & 86.4  & 69.7  & 72.4  & 133.2 & 83    & 81.1  & 121.4 & 121.3 & 29    \\
6593.87    & 26      & 2.44 & -2.42   & 120.4 & ---   &  ---  & 121.2 & ---   & 133.4 & 124.2 & ---   & ---   & 87.5  \\
6597.56    & 26      & 4.8  & -0.92   & 58.5  & 60.1  & 56.8  & 57.3  & 72.3  & 62.1  & 61.3  & 76.4  & 73.2  & 42.4  \\
6608.02    & 26      & 2.28 & -4.03   & 49.4  & 54.3  & 47.4  & 49.7  & 95.3  & 55.3  & 51.3  & 81.4  & 79.2  & 17.1  \\
6609.11    & 26      & 2.56 & -2.69   & 104.4 & 115.3 & 103.1 & 105.1 & ---   & 114.7 & 105.9 & 145.2 & 142   & 68.2  \\
6703.56    & 26      & 2.76 & -3.16   & 70.3  & 78.6  & 67.6  & 71.6  & 105.1 & 75.8  & 72.2  & 100.4 & 98.9  & 37.8  \\
6710.31    & 26      & 1.8  & -4.88   & 53.3  & 62.7  & 54.6  & 59.4  & ---   & 62.2  & ---   & 98.2  & ---   & 15.7  \\
6713.74    & 26      & 4.79 & -1.6    & 32.3  & 36.6  & 28.4  & 33.9  & 48.7  & 36.3  & 35.8  & 48.2  & 45.1  & 21.4  \\
6739.52    & 26      & 1.56 & -4.95   & 36.4  & 43.3  & 32.7  & 45.1  & 84    & 43.5  & 40.3  & 68.3  & ---   & 11.8  \\
6750.15    & 26      & 2.42 & -2.62   & 107.5 & 118.2 & 108.4 & 111.3 & ---   & 116.3 & 110.3 & 141.2 & 146   & 76.2  \\
6783.7     & 26      & 2.59 & -3.98   & 42.3  & 47.7  & 47.2  & 46    & ---   & ---   & ---   & 72.3  & 76.3  & 14.3  \\
6806.84    & 26      & 2.73 & -3.21   & 69.6  & 77.7  & 66.3  & 69.6  & 108.7 & 74.9  & 68.8  & 91.4  & 101.6 & 34    \\
6810.26    & 26      & 4.61 & -0.99   & 67.8  & 71.1  & 62.7  & 65.4  & 85.9  & 72.2  & 71.8  & 82.3  & 81.4  & 50    \\
6820.37    & 26      & 4.64 & -1.17   & 59    & 65.6  & 58.2  & 62.7  & 84.4  & 66.3  & 63    & 77.3  & 75.6  & 40.9  \\
6851.63    & 26      & 1.61 & -5.32   & 28.5  & 34.3  & ---   &  ---  & 64.3  & 26.9  & ---   & 48.6  & ---   & 6.7   \\
6858.15    & 26      & 4.61 & -0.93   & 67.8  & 73    & 66.8  & 70.3  & 84.3  & 73.2  & 72.3  & 81.1  & 79.4  & 50.2  \\
5159.05    & 26      & 4.28 & -0.65   & ---   & 84.3  &  ---  & ---   & ---   & 91.6  & 85.4  & ---   &  ---  & 68.6  \\
5916.24    & 26      & 2.45 & -2.99   & ---   & 98.8  & 86.3  & 90.4  & 138.2 & 98.1  & 92.4  & 124.2 & 125.9 & 53.3  \\
6120.24    & 26      & 0.91 & -5.95   & ---   & 32.2  & ---   & 25.6  & 76.2  & 30.1  & 28.4  & 60.7  & 64.4  & 5.1   \\
6551.67    & 26      & 0.99 & -5.79   & ---   & 35.5  & ---   & 30.6  & 72.8  & 30.5  & 29.9  & 63.3  & 61.8  & 6.1   \\
6752.7     & 26      & 4.64 & -1.2    & ---   & 62.1  & 52.8  & 64.7  & ---   & 60.4  & 51.7  & 70.6  & 83.7  & 38.2  \\
6793.25    & 26      & 4.07 & -2.47   & ---   & 29.3  & 23    & ---   & 44.3  & 30.8  & 28.9  & 40.5  & 44.1  & 13.2  \\
5717.83    & 26      & 4.28 & -0.979  & ---   & ---   & 83.3  & 92.4  & 104.2 & 95.3  & ---   & 105.5 & 102.3 & 63.1  \\
6436.4     & 26      & 4.19 & -2.46   & ---   & ---   & 21.3  & 28.6  & 46.7  & 25.8  & 23.9  & 40.4  & 36.6  & 11.1  \\
6646.93    & 26      & 2.61 & -3.99   & ---   & ---   & 31.7  & 34.9  &  ---  & 34.8  & 34.1  & ---   & 60.1  & 8.2   \\
6591.31    & 26      & 4.59 & -2.07   & ---   & ---   & ---   & 27.7  & 27.7  & 28.9  & 24.9  & 25.1  & ---   & 10.5  \\
6653.85    & 26      & 4.14 & -2.52   & ---   & ---   & ---   & ---   & 39.8  & 23.8  & 20.9  & 30.2  & 33.7  & 10.9  \\
6699.14    & 26      & 4.59 & -2.19   & ---   & ---   & ---   & ---   & ---   & 17.8  & 16.3  & 26.6  & 24.3  & 7.5   \\
6704.48    & 26      & 4.22 & -2.66   & ---   & ---   & ---   & ---   & ---   & 13.7  & 12.9  & 20.7  & 20.8  & 6.1   \\
6745.95    & 26      & 4.07 & -2.77   & ---   & ---   & ---   & ---   & ---   & ---   & 16.1  & ---   & 24.2  & 8.3   \\
4993.34    & 26.1    & 2.81 & -3.67   & 55.7  & 58.8  & 55.2  & 60.2  & 62.8  & 72.1  & 58.7  & 67.4  & ---   & 38    \\
5132.65    & 26.1    & 2.81 & -4      & 41.1  & 49.4  & 43.7  & ---   & 48.6  & 48.5  & 43.5  & 48.6  & 44.3  & 23.8  \\
5197.55    & 26.1    & 3.23 & -2.25   & 104.2 & ---   & ---   & ---   & ---   & ---   &  ---  & 112.6 & ---   & 81.9  \\
5234.61    & 26.1    & 3.22 & -2.24   & 106   & ---   & 110.3 & 109   & 100.2 & 105.3 & 105.7 & 108.3 & 106.5 & 81.9  \\
5284.09    & 26.1    & 2.89 & -3.01   & 82.5  & 87.1  & ---   & ---   &  ---  & 92    & 87.2  & 95.5  & 96.4  & 66.7  \\
5325.55    & 26.1    & 3.22 & -3.17   & 56.3  & 59.9  & 56    & 58.7  & 53.1  & ---   & 54.4  & 60.3  & 61.1  & 38.7  \\
5414.04    & 26.1    & 3.22 & -3.62   & 44.3  & 48    & 40.5  & 43.3  & 43.3  & 48.9  & 44.2  & 44.4  & 45.3  & 25.9  \\
5425.24    & 26.1    & 3.2  & -3.21   & 57.4  & 61.5  & 54.5  & 58.6  & 55.7  & 63.6  & 61.5  & 60.5  & ---   & 39.6  \\
5991.36    & 26.1    & 3.15 & -3.56   & 50.1  & 50.1  & 50.2  & 51.4  & 50.5  & 57.4  & 50.7  & 55.4  & ---   & 29.9  \\
6084.09    & 26.1    & 3.2  & -3.8    & 39.7  & 39.5  & 34.7  & 37.9  & 39.9  & 43.8  & 36.4  & 43.7  & ---   & 22.2  \\
6149.24    & 26.1    & 3.89 & -2.72   & 50.2  & 49    & 51.5  & 53.3  & 44.1  & 57.3  & 49.3  & 53.3  & 51    & 37.7  \\
6247.54    & 26.1    & 3.89 & -2.34   & 75    & 71.5  & 75.2  & 78.1  & 62.1  &  ---  & 68.7  & ---   & 66.4  & 55.9  \\
6416.92    & 26.1    & 3.89 & -2.68   & 55.7  & 57.4  & 56.9  & 55.4  & 52.2  & 58.7  & 52.5  & 56.9  & 56.3  & 39.6  \\
6432.68    & 26.1    & 2.89 & -3.58   &  ---  & 67.3  & 59.7  & ---   & ---   & 66.9  & 60.5  & 60.2  & 62.4  & 43.1  \\
4607.34    & 38      & 0    & 0.283   & 70.3  & 82.1  & 71.9  & 73.2  & 127.5 & 78.5  & 76.7  & 104.2 & 107.8 & 41    \\
5087.43    & 39.1    & 1.08 & -0.17   & 80.8  & 86.9  & 82.2  & 87.4  & 93.2  & 85.5  & 81.6  & 98.7  & 100.9 & 48.8  \\
5200.42    & 39.1    & 0.99 & -0.57   & 72.2  & 84.3  & 76.6  & ---   & 105.3 & 76.6  & 75.8  & 96.4  & 98.4  & 38.9  \\
5205.72    & 39.1    & 1.03 & -0.34   & 71.2  & ---   & ---   & ---   & ---   &  ---  & 76.9  & ---   & 101.1 & 41.4  \\
5289.82    & 39.1    & 1.03 & -1.85   & 20.4  & 23.3  & 18.9  & 27.5  & 42.2  & 22.1  & 19.4  & 29.7  & 31.3  & 5.2   \\
5402.78    & 39.1    & 1.84 & -0.44   & 34.6  & 43.3  & 36.8  & 43    & ---   & 37.3  & 37.8  & 50.3  & 50.7  & 13    \\
4883.68    & 39.1    & 1.08 & 0.07    & ---   & 102.8 & ---   & ---   & ---   & 99.2  & 95.2  & ---   & ---   & 60.1  \\
5385.13    & 40      & 0.52 & -0.64   & 13.3  & 10.8  & 12.4  & 10.6  & 46.5  & 10.1  & ---   & 29.4  & 34.6  & 1.9   \\
6127.46    & 40      & 0.15 & -1.06   & 18.4  & 19.8  & 18.2  & 19.3  & 65.1  & 15.5  & 17.4  & 42.3  & 45.4  & 3.8   \\
6134.57    & 40      & 0    & -1.28   & 15    & 13.2  & 17.4  & 12.7  & 59.8  & 11.1  & 13.7  & 39.4  & 38.3  & 2.2   \\
6143.18    & 40      & 0.07 & -1.1    &  ---  & ---   & 18.2  & 17.8  & 70.5  & 18.5  & 15.9  & 46.2  & 46.9  & 3     \\
5303.53    & 57.1    & 0.32 & -1.35   & 23.8  & 30.3  & 23.5  & 29.5  & 51.5  & 27.6  & 24.4  & 45.6  & 45.2  & 3.6   \\
5880.63    & 57.1    & 0.24 & -1.83   & 11.6  & 11.6  & 17    & 17.8  & 39    & 16.6  & 15.8  & 27.6  & 26.8  & 1.4   \\
6390.48    & 57.1    & 0.32 & -1.41   & 22.3  & 25.1  & 26    & 32    & 57.4  & 28.4  & 25.7  & 47.6  & 45.6  & 3.9   \\
4628.16    & 58.1    & 0.52 & -0.74   & 59.8  & 66.2  & 60    & 61.6  & 90.3  & 68.1  & 65.8  & 83.6  & 80.3  & 17.7  \\
5187.46    & 58.1    & 1.21 & 0.3     & 30.2  & 36.4  & 28    & 34.2  & 53.2  & 37.2  & 39.4  & 49.8  & 48.5  & 7.5   \\
5274.24    & 58.1    & 1.28 & 0.389   & 35.4  & 42.4  & ---   & 42.4  & 58.8  & 43.7  & 37.6  & 54.1  & 55.2  & 9.8   \\
5472.3     & 58.1    & 1.25 & -0.19   & 15.7  & 18.4  & ---   & 17.7  & 33.6  & 21.6  & 16.8  & ---   & 23.9  & 2.4   \\
4811.34    & 60.1    & 0.06 & -1.015  & 47    & 54.6  & 46.7  & 58.6  & 86.4  & 52.3  & 52.3  & 68.7  & 66.3  & 9.3   \\
4959.12    & 60.1    & 0.06 & -0.916  & 71.2  & ---   & 68.2  & 76.8  & 114.1 & 72.7  & 71.3  & 96.9  & 106   & 32.4  \\
5234.19    & 60.1    & 0.55 & -0.46   & 39.9  & ---   & ---   & 44.7  & ---   & ---   & ---   & ---   & ---   & 5.6   \\
5319.81    & 60.1    & 0.55 & -0.35   & 54.4  & 61.8  & 49.5  & 53.3  & 87.5  & 55.7  & 52.7  & 79.4  & ---   & 13    \\
5740.88    & 60.1    & 1.16 & -0.56   & 17.6  & 15.3  & 10    & 20.1  & 32    & 17.3  & 15.3  & 25.5  & 20.1  & 2.4   \\
5311.46$^{7}$  & 60.1  & 0.98 & -0.56   & ---   & 22.2  & ---   & 23.9  &  ---  &  ---  &  ---  & 32.1  & ---   & 2.3   \\
5130.59    & 60.1    & 1.3  & 0.1     & ---   &  ---  & ---   & ---   &  ---  & 43.6  &  ---  & ---   & ---   & 12.6  \\
\hline
\hline
\end{longtable}
\normalsize

==> NGC6633.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
\small
\begin{longtable}{cccccccccc}
\caption{List of absorption lines for NGC\,6633 stars}
\label{ngc6633}\\
\hline
\hline
Wavelength  & Species & $\chi$ & log g$f$ & E78   & E100  & E106  & E119  & E126  & Juno  \\
(\AA)       &         &   (eV) &         & (m\AA) & (m\AA)& (m\AA)&(m\AA) & (m\AA)&       \\
\hline
\hline
\endfirsthead
\endhead
5711.09    & 12      & 4.34 & -1.73    & 149.3 & 127.4 & 114.1 & 116   & 115.9 & 101.4 \\
6318.71    & 12      & 5.11 & -1.94    & 72.8  & 59.1  & 52.6  & 50.6  & 51.6  & 41.3  \\
7387.69    & 12      & 5.75 & -1.25    & 86.2  & 79.2  & 64.9  & 63.3  & 67.2  & 72.7  \\
8736.02    & 12      & 5.94 & -0.63    & 124.3 & ---   & ---   & 110.4 & 107.4 & 143.6 \\
4730.04    & 12      & 4.34 & -2.39    & ---   & 80.6  & 75.3  & 72.9  & 75.7  & 55.9  \\
6319.24    & 12      & 5.11 & -2.17    & ---   & 37.3  & 36.9  & 33.6  & 34.1  & 28.8  \\
8717.83    & 12      & 5.93 & -1.05    & ---   & 81.4  & 66.9  & 67.1  & 73.2  & 79.8  \\
7691.55    & 12      & 5.75 & -1       & ---   & ---   & ---   & 56.5  & 54.6  & 56.2  \\
6696.02    & 13      & 3.14 & -1.481   & 94.6  & 63.2  & 47.9  & 47.1  & 55.2  & 34.3  \\
6698.67    & 13      & 3.14 & -1.63    & 74.7  & 43.2  & 37.7  & 31.2  & 36.8  & 20.5  \\
7836.13    & 13      & 4.02 & -0.4     & 94.2  & 72.5  & 68.6  & 59.7  & 65.9  & 54.9  \\
8772.88    & 13      & 4.02 & -0.25    & 101.9 & 100.1 & 83.4  & ---   & 107.1 & 72.7  \\
7835.32    & 13      & 4.04 & 4.04     & ---   & 58.3  & 54.9  & 46.2  & 56.7  & 36.7  \\
8773.91    & 13      & 4.02 & -0.07    & ---   &  ---  & 126.1 & ---   & 126.3 & 93    \\
5488.98    & 14      & 5.61 & -1.69    &  37.4 &  37.6 &  36.2 &  ---  &  38.2  &  25.3     \\
5517.54    & 14      & 5.08 & -2.50    &  24.1 &  18.8 &  23.8 &  19.5 &  21.9  &  12.3     \\
5665.55    & 14      & 4.92 & -1.94    &  ---  &  66.3 &  63.3 &  58.6 &  62.1  &  40.6     \\
5684.48    & 14      & 4.95 & -1.55    &  80.3 &  75.7 &  72.5 &  67.7 &  75.1  &  61.1     \\
5690.43    & 14      & 4.93 & -1.77    &  65.7 &  68.7 &  67.5 &  54.9 &  ---   &  47.9     \\
6125.02    & 14      & 5.61 & -1.46    &  ---  &  45.0 &  45.7 &  38.2 &  43.8  &  31.5     \\
6142.48    & 14      & 5.62 & -1.29    &  40.9 &  40.1 &  44.3 &  37.4 &  41.6  &  34.1     \\
6145.02    & 14      & 5.62 & -1.31    &  49.9 &  48.3 &  42.9 &  40.2 &  45.8  &  37.5     \\
6243.82    & 14      & 5.62 & -1.24    &  48.5 &  51.1 &  60.9 &  58.1 &  57.6  &  42.1     \\
6244.47    & 14      & 5.62 & -1.09    &  65.9 &  51.8 &  53.6 &  53.5 &  60.1  &  42.0     \\
6414.98    & 14      & 5.87 & -1.03    &  44.8 &  58.5 &  53.0 &  52.3 &  52.3  &  45.1     \\
6721.85    & 14      & 5.86 & -1.12    &  ---  &  ---  &  ---  &  ---  &  57.8  &  42.5     \\
6741.63    & 14      & 5.98 & -1.43    &  ---  &  ---  &  ---  &  ---  &  23.9  &  14.1     \\
6848.58    & 14      & 5.86 & -1.52    &  ---  &  ---  &  ---  &  ---  &  26.4  &  16.5     \\
7003.57    & 14      & 5.96 & -0.94    &  ---  &  ---  &  ---  &  ---  &  ---   &  57.8     \\
5260.39    & 20	     & 2.52	& -1.72	&	83.5   &  60.5 &   51.8	&	---	  &	51.7	&	29.7	\\
5512.98    & 20	     & 2.93	& -0.46	&	131.7  & 112.2 &  107.2	&	96.8  &	104.2	&	83.7	\\
5581.97    & 20      & 2.52	& -0.56	&	 ---   & 129.1 &  116.4	&	112.1 &	118.3	&	92.5	\\
5590.11    & 20      & 2.52	& -0.57	&	144.1  & 122.1 &   ---  &	107.3 &	112.5	&	89.4	\\
5867.56    & 20      & 2.93	& -1.57	&	 78.0  &  ---  &   45.6	&	36.4  &	41.6	&	22.8	\\
6161.30    & 20      & 2.52	& -1.27	&	132.2  & 105.5 &   89.1	&	85.9  &	95.0	&	64.5	\\
6166.44    & 20      & 2.52	& -1.14	&	 80.9  & 104.2 &   95.4	&	93.4  &	92.9	&	70.5	\\
6169.04    & 20      & 2.52	& -0.80	&	 ---   & 125.4 &  112.2	&	109.2 &	114.9	&	89.3	\\
6169.56    & 20      & 2.53	& -0.48	&	 ---   & 139.7 &  130.3	&	129.6 &	137.7	&	110.0	\\
6455.60    & 20      & 2.52	& -1.34	&	128.9  &  98.4 &   89.0	&	84.0  &	86.0	&	54.6	\\
6471.66    & 20      & 2.53	& -0.69	&	 ---   & 130.7 &  122.3	&	115.7 &	124.5	&	89.1	\\
6493.78    & 20      & 2.52	& -0.11	&	 ---   &  ---  &    --- &	---   &   ---   &	122.2	\\
6499.65    & 20      & 2.52	& -0.82	&	 ---   &  ---  &  113.2	&	108.9 &   ---   &	87.2	\\
6572.78    & 20      & 0.00	& -4.24	&	 ---   &  ---  &   88.3	&	---   &   ---   &	29.9	\\
7326.15    & 20      & 2.93	& -0.21	&	 ---   &  ---  &   ---  &	131.3 &	135.8   &	108.2	\\
5022.87    & 22      & 0.83 & -0.43 &    ---   &  ---  &  111.4 &   ---   & 110.4   &   70.6    \\
5039.96    & 22      & 0.02 & -1.13 &    ---   &  ---  &   ---  &   ---	  & 114.5   &   71.1   \\
5064.65    & 22      & 0.05 & -0.99 &    ---   &  ---  &   ---  &   ---   & 128.7   &   85.2   \\
5113.45    & 22      & 1.44 & -0.78 &   115.2  &  68.1 &   ---  &   54.2  &  56.3   &   24.4   \\
5147.48    & 22      & 0.00 & -2.01 &    ---   &  ---  &   ---  &    ---  &  84.7   &   34.8   \\
5210.39    & 22      & 0.05 & -0.88 &    ---   &  ---  &  137.1 &    ---  & 133.4   &   88.2   \\
5219.70    & 22      & 0.02 & -2.29 &    ---   &  ---  &   ---  &    ---  &  72.0   &   28.2   \\
5295.77    & 22      & 1.07 & -1.63 &   104.2  &  48.2 &   41.6 &   37.7  &  36.2   &   12.6   \\
5866.45    & 22      & 1.07 & -0.84 &    ---   &  ---  &   ---  &   87.6  &  93.6   &   48.7   \\
6091.17    & 22      & 2.27 & -0.42 &    95.1  &  44.9 &   ---  &    ---  &  35.6   &   14.9   \\
6126.22    & 22      & 1.07 & -1.42 &   135.3  &  71.1 &   64.7 &    55.8 &  60.1   &   23.2   \\
6258.10    & 22      & 1.44 & -0.35 &    ---   &  97.1 &   90.9 &    84.2 &  87.8   &   51.0   \\
6261.10    & 22      & 1.43 & -0.48 &    ---   & 101.8 &   93.7 &    82.3 &  ---    &   48.9   \\
7138.91    & 22      & 1.44 & -1.59 &    ---   &  ---  &   ---  &     --- &  24.6   &    6.8   \\
5321.1     & 26      & 4.43 & -1.19    & 90.4  & 67.6  & 60.9  & 58    & 58.5  & 42.1  \\
5373.7     & 26      & 4.47 & -0.71    & 104   & 83.7  & 78    & 79.2  & 82    & 62.6  \\
5389.47    & 26      & 4.42 & -0.25    & 125.7 & 106.1 & 99.3  & 92    & 99.9  & 81.9  \\
5417.03    & 26      & 4.42 & -1.53    & 80.3  & 58.4  & 54.5  & 52.7  & 58.4  & 35.2  \\
5441.33    & 26      & 4.31 & -1.58    & 81.1  & 55.6  & 55.8  & 48.8  & 51.5  & 31.5  \\
5445.04    & 26      & 4.39 & 0.041    & 154.8 & 139.7 & 135.2 & 130.6 & 133.7 & 122.2 \\
5560.21    & 26      & 4.43 & -1.04    & 94.8  & 73.5  & 69.9  & 61.7  & 67.4  & 51.1  \\
5584.76    & 26      & 3.57 & -2.17    & 98.4  & 70.6  & 65.9  & 58    & 62.9  & 39.2  \\
5624.02    & 26      & 4.39 & -1.33    & 103.1 & 78.6  & ---   & 75.7  & 72.2  & 52.3  \\
5633.94    & 26      & 4.99 & -0.12    & 101.3 & 84.8  & 83    & 83.5  & 86.7  & 65.2  \\
5635.82    & 26      & 4.26 & -1.74    & 78.9  & ---   & 54.3  & 49    & 51.9  & 34    \\
5638.26    & 26      & 4.22 & -0.72    & 128.5 & 103.7 & 97.4  & 95.8  & 97.3  & 77.4  \\
5705.46    & 26      & 4.3  & -1.36    & 82.5  & 64.9  & 59.9  & 58.9  & 60.7  & 38.8  \\
5717.83    & 26      & 4.28 & -0.979   & 111.4 & 91.7  & 93.5  & 83.6  & 94.5  & 63.1  \\
5731.76    & 26      & 4.26 & -1.15    & 104.9 & 88.7  & 83.5  & 77    & 86.3  & 57.4  \\
5916.24    & 26      & 2.45 & -2.99    & 147.3 & 105.8 & 99.5  & 88.6  & 92.8  & 53.3  \\
6024.05    & 26      & 4.55 & -0.06    & 149.7 & 132.3 & 128.3 & 123.2 & 125.4 & 110.4 \\
6027.05    & 26      & 4.08 & -1.09    & 113.2 & 96.9  & 91.8  & 86.4  & 91.8  & 62.5  \\
6056       & 26      & 4.73 & -0.4     & 107   & 90.8  & 94.1  & 82.9  & 83.6  & 71.1  \\
6079       & 26      & 4.65 & -0.97    & 85    & 69.9  & 64.5  & 62    & 61.7  & 47.4  \\
6093.64    & 26      & 4.61 & -1.35    & 71.4  & 55.7  & 49.5  & 46.5  & 53.6  & 30.1  \\
6096.66    & 26      & 3.98 & -1.78    & 87.1  & 67    & 64.3  & 55.9  & 60.8  & 37.2  \\
6120.24    & 26      & 0.91 & -5.95    & 91.4  & 38.5  & 31.4  & 25.3  & 27.4  & 5.1   \\
6151.61    & 26      & 2.18 & -3.29    & 144.3 & 97.7  & 87.9  & 82.6  & 87.7  & 49.2  \\
6165.36    & 26      & 4.14 & -1.47    & 95.8  & 76.5  & 70.1  & 65.2  & 68    & 44    \\
6187.99    & 26      & 3.94 & -1.57    & 101.8 & 80.5  & 73.6  & 70.4  & 68.7  & 47.7  \\
6380.74    & 26      & 4.19 & -1.32    & 108.7 & 87.7  & 88.4  & 73.7  & 74.3  & 53.8  \\
6419.95    & 26      & 4.73 & -0.09    & 128.7 & 108.9 & 103.1 & 97.3  & 98.3  & 87    \\
6597.56    & 26      & 4.8  & -0.92    & 85.3  & 68.2  & 65.3  & 57.2  & 59.9  & 42.4  \\
6608.02    & 26      & 2.28 & -4.03    & 103.8 & 56.5  & 52.2  & 44.1  & 47.2  & 17.1  \\
6609.11    & 26      & 2.56 & -2.69    & 164.4 & 117.9 & 108.1 & 98.8  & 105.6 & 68.2  \\
6699.14    & 26      & 4.59 & -2.19    & 28    & 18    & 21.7  & 12.1  & 17.2  & 7.5   \\
6703.56    & 26      & 2.76 & -3.16    & 122.6 & 85.7  & 78.1  & 66.4  & 75.9  & 37.8  \\
6704.48    & 26      & 4.22 & -2.66    & 28.5  & 18.9  & 15.4  & 11.3  & 13.8  & 6.1   \\
6710.31    & 26      & 1.8  & -4.88    & 116.3 & 67.6  & 63.5  & 52.4  & 55.8  & 15.7  \\
6713.74    & 26      & 4.79 & -1.6     & 51.5  & 41.2  & 38.6  & 36.7  & 38.3  & 21.4  \\
6739.52    & 26      & 1.56 & -4.95    & 101.6 & 54.8  & 51.4  & 35.6  & 36.7  & 11.8  \\
6745.95    & 26      & 4.07 & -2.77    & 33.5  & ---   & ---   &  ---  &  ---  & 8.3   \\
6806.84    & 26      & 2.73 & -3.21    & 115.9 & 82.1  & 73.7  & 61.9  & 71    & 34    \\
6810.26    & 26      & 4.61 & -0.99    & 90.2  & 77.6  & 70    & 62.1  & 69.8  & 50    \\
6820.37    & 26      & 4.64 & -1.17    & 89.1  & 68.4  & 62.9  & 60.8  & 64.1  & 40.9  \\
6851.63    & 26      & 1.61 & -5.32    & 88.5  & 39.4  & 35    & 25.7  & 31.3  & 6.7   \\
6858.15    & 26      & 4.61 & -0.93    & 88.9  & 73.9  & 73.4  & 63.4  & 70.8  & 50.2  \\
7132.98    & 26      & 4.08 & -1.61    & 96    & 75.2  & 71.8  & 64.4  & 73.3  & 42.5  \\
5242.49    & 26      & 3.63 & -0.97    &  ---  & 116.7 & 110.8 & 108.2 & 109.3 & 85.9  \\
5253.03    & 26      & 2.28 & -3.79    &  ---  & 51.2  & 45.1  & 42.5  & 40.7  & 17.1  \\
5288.52    & 26      & 3.69 & -1.51    &  ---  & 91.6  & 94.1  & 82.2  & 93.1  & 58.6  \\
5322.04    & 26      & 2.28 & -2.84    &  ---  & 109.3 & 100.8 & 96.8  & 97.7  & 62.1  \\
5364.87    & 26      & 4.45 & 0.23     &  ---  & 137.9 & 144.9 & 134.8 & 137.4 & 132.9 \\
5367.46    & 26      & 4.42 & 0.439    &  ---  & 146.2 & 146.4 & 142.2 & 144.5 & 145.1 \\
5410.91    & 26      & 4.47 & 0.4      &  ---  & 133.8 & 133.4 & 126.9 & 131   & 130.9 \\
5691.49    & 26      & 4.3  & -1.37    &  ---  & 75.6  & 69    & 62.6  & 64.4  & 40.7  \\
5852.21    & 26      & 4.55 & -1.18    &  ---  & 71.9  & 70.2  & 57.2  & 65.4  & 39.9  \\
5883.81    & 26      & 3.96 & -1.21    &  ---  & 97.4  & 91.9  & 81.9  & 88.4  & 70.5  \\
6157.72    & 26      & 4.08 & -1.11    &  ---  & 99.1  & 96.8  & 92.4  & 96.4  & 63.5  \\
6173.33    & 26      & 2.22 & -2.88    &  ---  & 120.4 & 112.3 & 100.5 & 107.1 & 67.7  \\
6200.31    & 26      & 2.61 & -2.44    &  ---  & 117.3 & 110.8 & 104.9 & 104.2 & 71.7  \\
6322.68    & 26      & 2.59 & -2.43    &  ---  & 124.5 & 114.1 & 108.3 & 111.4 & 78.6  \\
6392.53    & 26      & 2.28 & -4.03    &  ---  & 56.3  & 50.2  & 40.5  & 44.7  & 18.2  \\
6574.22    & 26      & 0.99 & -5.02    &  ---  & 89.3  & 77    & 66.8  & 77.8  & 29    \\
6750.15    & 26      & 2.42 & -2.62    &  ---  & 126.5 & 112.6 & 109.4 & 115.6 & 76.2  \\
6752.7     & 26      & 4.64 & -1.2     &  ---  & 69.3  & 64.8  & 65.4  & 68.4  & 38.2  \\
5522.44    & 26      & 4.21 & -1.4     &  ---  & ---   & 71.1  & 56.7  & 65.4  & 45.1  \\
5554.89    & 26      & 4.55 & -0.38    &  ---  & ---   & 120.6 & 116.4 & 121.2 & 100.1 \\
6646.93    & 26      & 2.61 & -3.99    &  ---  & ---   & 36.5  & 28    & 33.7  & 8.2   \\
4993.34    & 26.1    & 2.81 & -3.67    & 63.5  & ---   & 62.9  & 54.1  & 60.3  & 38    \\
5234.61    & 26.1    & 3.22 & -2.24    & 106.2 & 112.4 & 109.1 & 102.7 & 104.9 & 81.9  \\
5325.55    & 26.1    & 3.22 & -3.17    & 57.1  & 66.8  & 59.3  & 60.7  & 66.3  & 38.7  \\
5414.04    & 26.1    & 3.22 & -3.62    & 43.5  & 52.3  & 49.8  & 41.7  & 43.2  & 25.9  \\
5425.24    & 26.1    & 3.2  & -3.21    & 58.3  & 66    & 67.2  & 57.2  & 59.2  & 39.6  \\
5991.36    & 26.1    & 3.15 & -3.56    & 49.3  & 58.9  & 55.6  & 55.3  & 57.5  & 29.9  \\
6084.09    & 26.1    & 3.2  & -3.8     & 37.2  & 46.1  & 45.4  & 40.1  & ---   & 22.2  \\
6149.24    & 26.1    & 3.89 & -2.72    & 47.5  & 55.2  & 54.1  & 53.4  & 52.1  & 37.7  \\
6247.54    & 26.1    & 3.89 & -2.34    & 63.3  & 74.8  & 81.7  & 72.8  & 73.5  & 55.9  \\
6432.68    & 26.1    & 2.89 & -3.58    & 64.5  & 72.5  & 66.4  & 58.9  & 67.5  & 43.1  \\
5132.65    & 26.1    & 2.81 & -4       & ---   & 51.7  & 52.8  & 45.2  & 46.1  & 23.8  \\
5197.55    & 26.1    & 3.23 & -2.25    & ---   & 108.7 & ---   & 109.2 & 109.3 & 81.9  \\
5284.09    & 26.1    & 2.89 & -3.01    & ---   & 93    & ---   & 88.9  & 89.7  & 66.7  \\
6416.92    & 26.1    & 3.89 & -2.68    & ---   & 59.7  & 59.2  & 53.4  & 58    & 39.6  \\
4607.34    & 38      & 0    & 0.283    & 130.9 & 88.4  & 81.5  & 78.1  & 82.1  & 41    \\
4883.68    & 39.1    & 1.08 & 0.07     & 129.1 & 100.6 & 97.4  & 94.8  & 92.9  & 60.1  \\
5200.42    & 39.1    & 0.99 & -0.57    & 111.9 & 84.6  & 78.5  & 74.4  & 78.1  & 38.9  \\
5289.82    & 39.1    & 1.03 & -1.85    & 44.1  & 23.6  & 20.8  & 20.2  & 21    & 5.2   \\
5402.78    & 39.1    & 1.84 & -0.44    & 53.7  & 44.7  & 38.6  & 36.6  & 33.6  & 13    \\
5087.43    & 39.1    & 1.08 & -0.17    & ---   & 92.3  & 77    & 82.4  & 83.1  & 48.8  \\
5385.13    & 40      & 0.52 & -0.64    & 55.3  & ---   & ---   & 6.1   & 7     & 1.9   \\
6134.57    & 40      & 0    & -1.28    & 79.9  & 13.3  & 10.2  & 7.5   & 10.9  & 2.2   \\
6143.18    & 40      & 0.07 & -1.1     & 87.5  & 19.5  & 14.3  & 12.1  & 13.6  & 3     \\
6127.46    & 40      & 0.15 & -1.06    &  ---  & 22.8  & 10.8  & 11.5  & 12.8  & 3.8   \\
5303.53    & 57.1    & 0.32 & -1.35    & 53.6  & 30    & 25.3  & 20.6  & 21.5  & 3.6   \\
5880.63    & 57.1    & 0.24 & -1.83    & 41.4  & 13.9  & ---   & ---   & 9.8   & 1.4   \\
6390.48    & 57.1    & 0.32 & -1.41    & 68.7  & 34.3  & 27.3  & 18.4  & 27.2  & 3.9   \\
5187.46    & 58.1    & 1.21 & 0.3      & 58.9  & 32.2  & 31.3  & 21.7  & 23.5  & 7.5   \\
5274.24    & 58.1    & 1.28 & 0.389    & 64.5  & 43.1  & 32    & 30.8  & 31.1  & 9.8   \\
5472.3     & 58.1    & 1.25 & -0.19    & 30.4  & 14.2  & 14    & 7.1   & 11    & 2.4   \\
4628.16    & 58.1    & 0.52 & -0.74    & ---   & 63.2  & ---  & ---   & ---   & 17.7  \\
4811.34    & 60.1    & 0.06 & -1.015   & 90    & 57.9  & 45.3  & 35.4  & 40.8  & 9.3   \\
4959.12    & 60.1    & 0.06 & -0.916   & 126.5 & 88.3  & 70.6  & 63.3  & 70.6  & 32.4  \\
5234.19    & 60.1    & 0.55 & -0.46    & 65.1  & 43.1  & 36.8  & 21.1  & ---   & 5.6   \\
5319.81    & 60.1    & 0.55 & -0.35    & 88.3  & 64.9  & ---   & ---   & ---   & 13    \\
5740.88    & 60.1    & 1.16 & -0.56    & 30.6  & 21.1  & ---   & ---   & 11.1  & 2.4   \\
5130.59    & 60.1    & 1.3  & 0.1      & ---   & ---   & ---   & 30.6  & ---   & 12.6  \\
5311.46$^{7}$ & 60.1    & 0.98 & -0.56    & ---   & ---   & ---   & ---   & 11.8  & 2.3   \\
\hline
\hline
\end{longtable}
\normalsize

==> NGC6940.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
\small
\begin{longtable}{ccccccccccccccccc}
\caption{List of absorption lines for NGC\,6940 stars}
\label{ngc6940}\\
\hline
\hline
Wavelength  & Species & $\chi$ & log g$f$ & E28   & E30    & E67    & E87    & E101   & E105   & E108   & E132   & E138   &  E139  & E152   & Juno \\
(\AA)       &         &   (eV) &         & (m\AA) & (m\AA) & (m\AA) & (m\AA) & (m\AA) & (m\AA) & (m\AA) & (m\AA) & (m\AA) & (m\AA) & (m\AA) &       \\
\hline
\hline
\endfirsthead
%
\endhead
%
5711.09       & 12         & 4.34  & -1.73    & 129   & 135   & 134.2 & 121.6 & 131.6 & 138   & 117.5 & 131.9 & 125.9 & 128.6 & 130.6 & 101.4   \\
6318.71       & 12         & 5.11  & -1.94    & 53.5  & 64.5  & 64.9  & 60.9  & 58.7  & 64.8  & 56.9  & 67.5  & 55.5  & 65.8  & 63.5  & 41.3    \\
8712.69       & 12         & 5.93  & -1.31    & 70.5  & ---   & ---   & ---   & 69.9  & 75.7  & 56.2  & 86.4  & 72.3  & ---   & 88    & 52.8    \\
8717.83       & 12         & 5.93  & -1.05    & 101.4 & 90.5  & ---   & ---   & 114.1 & 98.4  & ---   & 110.2 & ---   & 100.9 & 93.7  & 79.8    \\
8736.02       & 12         & 5.94  & -0.63    & 140.4 & 150   & 144.7 & ---   & ---   & 139.5 & ---   & 148.9 & ---   & 147.1 & 146.7 & 143.6   \\
7387.69       & 12         & 5.75  & -1.25    & ---   & 90    & 90.7  & 87.2  & 93.2  & 89.3  & 88.8  & 96.2  & 82.6  & 96.1  & 97.4  & 72.7    \\
7691.55       & 12         & 5.75  & -1       & ---   & 95.2  & 80.3  & 100.1 & 99.6  & 105.9 & ---   & ---   & 83.2  & ---   & 100.1 & 56.2    \\
6319.24       & 12         & 5.11  & -2.17    & ---   & ---   & ---   & ---   & ---   & ---   & 43.7  & ---   & ---   & ---   & ---   & 28.8    \\
6696.02       & 13         & 3.14  & -1.481   & 58.3  & ---   & ---   & 63.6  & ---   & ---   & ---   & ---   & ---   & ---   & ---   & 34.3    \\
6698.67       & 13         & 3.14  & -1.63    & 43.1  & 54.6  & 50    & 42.4  & 55.5  & 60.9  & 38    & 55.5  & 48.6  & 51.3  & 54.1  & 20.5    \\
7835.32       & 13         & 4.04  & -0.58    & 56.1  & ---   & ---   & 57.6  & ---   & ---   & ---   & ---   &  ---  & ---   & ---   & 36.7    \\
7836.13       & 13         & 4.02  & -0.4     & 70.1  & 79.2  & 76.6  &  ---  & 82.2  & 88.4  & 65.9  & 82.8  & 67.4  & 76.1  & 81.1  & 54.9    \\
8772.88       & 13         & 4.02  & -0.25    & 90.5  &  ---  &  ---  &  ---  &  ---  &  ---  & ---   & ---   &  ---  &  ---  &  ---  & 72.7  \\
8773.91       & 13         & 4.02  & -0.07    & 113.1 &  ---  &  ---  &  ---  &  ---  &  ---  & ---   & ---   &  ---  &  ---  &  ---  & 93.0  \\
5488.98       & 14         & 5.61  & -1.69    &  39.8 &	 ---  &	 43.5 &	 45.4 &	 ---  &	 43.7 &	26.7  &	47.9  &  ---  &  44.8 &	 45.7 & 25.3  \\
5517.54       & 14         & 5.08  & -2.50    &  ---  &  30.3 &	 ---  &	 34.2 &	 ---  &  33.6 &	21.8  &	32.8  &  ---  &  ---  &  ---  & 12.3  \\
5665.55       & 14         & 4.92  & -1.94    &  65.3 &  73.1 &  ---  &  69.1 &  73.4 &  72.7 & 60.2  & 74.1  &  62.2 &  65.4 &  74.1 & 40.6  \\
5684.48       & 14         & 4.95  & -1.55    &  83.3 &  80.2 &  ---  &  80.1 &  ---  &  ---  &  ---  &  ---  &  ---  &  ---  &  ---  & 61.1  \\
5690.43       & 14         & 4.93  & -1.77    &  66.8 &  70.9 &  79.3 &  69.7 &  78.3 &  ---  & 59.5  & 81.7  &  ---  &  ---  &  78.2 &	47.9  \\
6125.02       &	14         & 5.61  & -1.46    &  49.1 &  48.9 &  49.3 &  49.3 &  55.7 &  50.2 & 43.8  & 57.8  &  45.9 &	 ---  &	 53.5 & 31.5  \\
6142.48       & 14         & 5.62  & -1.29    &  ---  &  52.2 &  49.0 &  ---  &  ---  &  52.3 & 40.3  &	 ---  &  48.9 &	 ---  &	 ---  & 34.1  \\
6145.02       & 14         & 5.62  & -1.31    &  48.9 &  ---  &  60.1 &  53.3 &  58.8 &  58.6 &	---   & 65.2  &  51.7 &  55.4 &  57.6 & 37.5   \\
6243.82       & 14         & 5.62  & -1.24    &  60.2 &  67.2 &  ---  &  57.4 &  63.9 &  71.7 & 54.6  & ---   &  56.6 &  ---  &  67.1 & 42.1   \\
6244.47       & 14         & 5.62  & -1.09    &  62.6 &  63.1 &  ---  &  56.8 &  68.9 &  67.5 & 55.8  & 71.7  &  56.3 &  60.9 &  65.8 & 42.0   \\
6414.98       & 14         & 5.87  & -1.03    &  ---  &  ---  &  ---  &  ---  &  ---  &  ---  &  ---  &  ---  &   --- &  ---  &  63.9 &	45.1   \\
6721.85       & 14         & 5.86  & -1.12    &  60.7 &  63.6 &  66.4 &  65.7 &  63.6 &  68.1 &  55.1 & 74.2  &  60.9 &  66.6 &  68.1 & 42.5   \\
6741.63       & 14         & 5.98  & -1.43    &  ---  &  ---  &  ---  &  ---  &  ---  &	 ---  &  ---  &  ---  &   --- &  ---  &  25.2 & 14.1   \\
6848.58       &	14         & 5.86  & -1.52    &  ---  &  ---  &  ---  &  ---  &  ---  &  ---  &  ---  & 35.8  &  29.5 &  31.2 &  ---  & 16.5   \\
7003.57       & 14         & 5.96  & -0.94    &  65.5 &  ---  &  ---  &  ---  &  ---  &  ---  &  ---  &  ---  &  ---  &  ---  &  ---  & 57.8    \\
5260.39       & 20         & 2.52  & -1.72    &  60.4 &  65.9 &  61.5 &  64.2 &  ---  &  ---  &  44.0 &  ---  &  ---  &  ---  &  ---  & 29.7   \\
5512.98       &	20         & 2.93  & -0.46    & 105.5 & 119.5 &	112.5 &  ---  &	114.9 &	122.9 & 106.1 & 119.0 & 106.5 & 112.1 & 119.6 & 83.7   \\
5581.97       &	20         & 2.52  & -0.56    &	120.9 & 130.2 &	128.6 & 126.5 & 134.2 &	140.7 &	118.5 &	134.8 &	121.2 &	126.9 &	135.9 & 92.5  \\
5590.11       &	20         & 2.52  & -0.57    &  ---  & 132.2 &	128.0 & 123.5 &  ---  &  ---  &  ---  &  ---  &  ---  &  ---  &  ---  & 89.4  \\
5867.56       & 20         & 2.93  & -1.57    &  46.8 &  54.6 &  56.1 &  52.8 &  55.9 &  61.5 &  ---  &  60.2 &  44.7 &  51.2 &  59.4 & 22.8  \\
6161.30       & 20         & 2.52  & -1.27    &  95.8 & 116.9 & 101.0 & 101.3 &	111.5 & 113.6 &	85.0  &	117.2 &  97.5 &	103.7 &	109.2	&	64.5	\\
6166.44       & 20         & 2.52  & -1.14    & 101.0 & 109.6 & 111.0 & 103.9 &	109.3 & 118.9 &	89.1  &  ---  &  98.4 &	106.8 &	114.9	&	70.5	\\
6169.04       & 20         & 2.52  & -0.80    & 117.3 & 128.5 & 126.4 & 123.9 &	126.5 &	137.1 &	111.6 &	137.3 &	117.1 &	127.6 &	131.2	&	89.3	\\
6169.56       &	20         & 2.53  & -0.48    & 135.3 &	149.2 & 139.3 &	 ---  & ---   & ---   & 129.7 &  ---  & 134.8 &	144.8 & ---     &	110.0	\\
6455.60       & 20         & 2.52  & -1.34    &  90.5 &	 ---  &	100.1 &  94.9 &	102.5 & 108.6 &	 78.9 &	107.3 &	 88.2 &	 94.6 &	102.6	&	54.6	\\
6471.66       & 20         & 2.53  & -0.69    & 122.8 & 137.2 &	135.1 & 128.3 &	130.4 &	 ---  &	125.1 &	136.9 &	121.1 &	128.4 &	138.1	&	89.1	\\
6493.78       &	20         & 2.52  & -0.11    &	 ---  &	 ---  &	 ---  &	 ---  &	 ---  &	 ---  &	 ---  &	 ---  &  ---  &	 ---  &  ---    &	122.2	\\
6499.65       &	20         & 2.52  & -0.82    &	122.7 &	 ---  & 129.8 &	124.2 &	130.6 &	139.6 &	 ---  &	136.6 &	120.7 &	128.7 &	134.8   &   87.2	\\
6572.78       & 20         & 0.00  & -4.24    &  ---  &  ---  &  ---  &  ---  &  ---  &	 ---  &  ---  &	112.8 &  97.2 & 106.2 &	119.4	&	29.9	\\
7326.15       & 20         & 2.93  & -0.21    &  ---  &	 ---  &  ---  &  ---  &  ---  &  ---  &	123.1 &  ---  &  ---  &  ---  &	150.6	&	108.2	\\
5022.87       & 22         & 0.83  & -0.43    &	118.2 & 124.8 & 126.0 &  ---  & 119.0 & 136.7 &  ---  &  ---  &	114.1 &	115.4 &	 ---    &	70.6   \\
5039.96       & 22         & 0.02  & -1.13    &	120.6 & 140.2 & 126.3 & 126.9 &	128.4 &  ---  & 118.9 &	128.9 &	122.3 &	127.8 &  ---    &   71.1    \\
5064.65       & 22         & 0.05  & -0.99    & 128.9 &	 ---  & 144.1 &  ---  &  ---  &  ---  &  ---  &	149.7 &	134.3 &	148.5 &  ---    &   85.2	\\
5113.45       & 22         & 1.44  & -0.78    &  ---  &  ---  &  ---  &  ---  &  ---  &  83.9 &  ---  &  ---  &  ---  &  ---  &  75.4   &	24.4	\\
5147.48       &	22         & 0.00  & -2.01    &  84.2 & 105.3 &  95.6 &  93.5 &  ---  & 114.1 &  80.8 & 102.7 &  ---  &  92.2 &  102.5  &   34.8  \\
5210.39       &	22         & 0.05  & -0.88    &  ---  &  ---  &  ---  &  ---  & 145.3 &	 ---  &  ---  &	150.6 &	143.0 &	144.3 &  ---    &   88.2	\\
5219.70       & 22         & 0.02  & -2.29    &  84.7 & 104.2 &  96.9 &  87.8 &  87.8 & 110.8 &  77.1 &  92.1 &  90.4 &	 86.6 &	 99.8	&	28.2	\\
5295.77       & 22         & 1.07  & -1.63    &  43.2 &  52.7 &  50.5 &  50.1 &  49.7 &  67.6 &  34.7 &  54.3 &  49.6 &  50.1 &	 55.1	&	12.6	\\
5866.45       & 22         & 1.07  & -0.84    &  91.4 &	115.6 & 103.8 &	100.3 & 110.3 &	131.1 &  93.7 & 110.7 &	108.6 &	101.8 &	122.3	&	48.7	\\
6091.17       & 22         & 2.27  & -0.42    &  50.0 &  60.1 &  52.3 &  48.8 &  50.5 &	 64.2 &  31.2 &  52.7 &  44.4 & 46.5  &	 57.8   &	14.9	\\
6126.22       & 22         & 1.07  & -1.42    &  67.5 &  78.2 &  76.0 &  73.4 &  75.9 &  96.3 &  ---  &  79.1 &  73.6 &  66.1 &  79.4   &   23.2    \\
6258.10       &	22         & 1.44  & -0.35    &  ---  & 104.1 &  ---  &  ---  &  ---  &  ---  &  ---  & 103.2 &  ---  &  95.4 &  ---    &	51.0	\\
6261.10       & 22         & 1.43  & -0.48    & 100.1 &	118.7 &	112.7 &	 ---  & 108.8 & 139.5 &  90.7 &	117.3 &  99.0 &	105.9 & 121.5	&	48.9	\\
5242.49       & 26         & 3.63  & -0.97    & 119.8 & 121.9 & 117   & 120.3 & 118.8 & 123.4 & 111.2 & 121.2 & 117.7 & 116.7 & 120.2 & 85.9    \\
5253.03       & 26         & 2.28  & -3.79    & 50.4  & 66.3  & 57.9  & 59.4  & 57.8  & 65    & 39.8  & 63.5  & 51.4  & 59.9  & 64.3  & 17.1    \\
5288.52       & 26         & 3.69  & -1.51    & 89.8  & 96.4  & 98.5  & 86.7  & 94.3  & 109.5 & 100.2 & 101.9 & 93.2  & 92.4  & 104.2 & 58.6    \\
5321.1        & 26         & 4.43  & -1.19    & 63.5  & 70.9  & 73.4  & 72.4  & 67    & 74.1  & 75.4  & 71.4  & 65.5  & 68.2  & 69.5  & 42.1    \\
5322.04       & 26         & 2.28  & -2.84    & 101.5 & 115.9 & 108.5 & 105.3 & 105.8 & 120.7 & 98.2  & 110.7 & 103.3 & 101.4 & 114.6 & 62.1    \\
5364.87       & 26         & 4.45  & 0.23     & 139.7 & 142.7 & 147.6 & 133.5 & 146.5 & 143.1 & 139.2 & 145.2 & 134.2 & 143.1 & 144.9 & 132.9   \\
5367.46       & 26         & 4.42  & 0.439    & 141.9 & 146.2 & ---   & 147.9 & 148.8 & 150.1 & 146.5 & 149.3 & 148.2 & 145.6 & ---   & 145.1   \\
5373.7        & 26         & 4.47  & -0.71    & 81.3  & 87.5  & 89.4  & 91.2  & 87.7  & ---   & 88.1  & 88    & 82.5  & 84.7  & 94.8  & 62.6    \\
5389.47       & 26         & 4.42  & -0.25    & 101.5 & 106.8 & 105.8 & 100.5 & 104.9 & 112   & ---   & 107.5 & 100.1 & 104.2 & 109.3 & 81.9    \\
5410.91       & 26         & 4.47  & 0.4      & 137.8 & 139.3 & 135.2 & 131.7 & ---   & ---   & ---   & 138.5 & 134   & 137.3 & ---   & 130.9   \\
5417.03       & 26         & 4.42  & -1.53    & 59.7  & 59.6  & 59.9  & 68.4  & 55.8  & 64.6  & 52.2  & 63.7  & 57.6  & 56.1  & 61.9  & 35.2    \\
5441.33       & 26         & 4.31  & -1.58    & 61.2  & 63.8  & 62.9  & 64.3  & 63.6  & 68.5  & 59    & 64.6  & 55.9  & 55.6  & 62.7  & 31.5    \\
5445.04       & 26         & 4.39  & 0.041    & 130.8 & 141.1 & ---   & 135.2 & 134.8 & 142.4 & 136   & 135.1 & 132.3 & 134.1 & 140.6 & 122.2   \\
5522.44       & 26         & 4.21  & -1.4     & 69.1  & 72.1  & 78.1  & 72.3  & 65.9  & 76.4  & 61.3  & 72.4  & 66.5  & 69.6  & 76.6  & 45.1    \\
5554.89       & 26         & 4.55  & -0.38    & 123.9 & 138.1 & 133.3 & 127.7 & 134.1 & 137.8 & 120   & 137.1 & 123.1 & 128.5 & 137.8 & 100.1   \\
5560.21       & 26         & 4.43  & -1.04    & 69.7  & 77.6  & 73.2  & 71.2  &  ---  & 78.3  & 72.5  & 77.1  & 70.8  & 72.3  & 76.1  & 51.1    \\
5584.76       & 26         & 3.57  & -2.17    & 67.2  & 84.3  & 70.1  & 72.6  & 79.1  & ---   &  ---  & 80.7  & 76.6  & 76.7  & 79.6  & 39.2    \\
5624.02       & 26         & 4.39  & -1.33    & 72.6  & 91.5  & 81.7  & 79.2  & 74.3  & 78.2  & 75.1  & 83.9  & 72.8  & ---   & 87.2  & 52.3    \\
5633.94       & 26         & 4.99  & -0.12    & 82.1  & 92.6  & 88.9  & 90.5  & 89    & 90.5  & 79.3  & 92.4  & 84    & ---   & 91.1  & 65.2    \\
5635.82       & 26         & 4.26  & -1.74    & 58.8  & 61.4  & 57.6  & ---   & 64.6  & 63.8  & 46.4  & 57.8  & 54.9  & 55    & 59.4  & 34      \\
5638.26       & 26         & 4.22  & -0.72    & 103.4 & 104.7 & 102.1 & 100.2 & 106.5 & 111.2 & 95.7  & 107.6 & 98.4  & 107.2 & 109.9 & 77.4    \\
5691.49       & 26         & 4.3   & -1.37    & 71.6  & 80.6  & 73.3  & 71.5  & 78.1  & 86.2  & 74.2  & 83.1  & 72.1  & 77.7  & 83.4  & 40.7    \\
5705.46       & 26         & 4.3   & -1.36    & 68.7  & 73.5  & 72    & 72.1  & 63.5  & 76.3  & 59.2  & 69.8  & 60.1  & 61.4  & 72.9  & 38.8    \\
5717.83       & 26         & 4.28  & -0.979   & 95.4  & 109.9 & 101.9 & 91.8  & ---   & ---   & 101.3 & 105.5 & 95.3  & 98.4  & 107   & 63.1    \\
5731.76       & 26         & 4.26  & -1.15    & 82.7  & 83.9  & 86.6  & 88.9  & 86.6  & 89.9  & 85.7  & 89    & 80.1  & 84.1  & 86.8  & 57.4    \\
5806.72       & 26         & 4.61  & -0.9     & 80.9  & 83.6  & 76.9  & 77.8  & 81    & 86.8  & 73.9  & 85.1  & 73.4  & 79    & 86.3  & 53.9    \\
5814.8        & 26         & 4.28  & -1.82    & 50    & 44.4  & 45.3  & 47.4  & 43    & 50.9  & 33.7  & 50.5  & 44.7  & 42.3  & 48.1  & 23.4    \\
5852.21       & 26         & 4.55  & -1.18    & 62.5  & 79.5  & 73.8  & 75    & 70.1  & 83.9  & 59    & 72.5  & 66.2  & 72.8  & 78.6  & 39.9    \\
5883.81       & 26         & 3.96  & -1.21    & 93.9  & 104.4 & 98.7  & 93.8  & 93.4  & 107.1 & 102.9 & 104.6 & 91.1  & 102.7 & 104.5 & 70.5    \\
5916.24       & 26         & 2.45  & -2.99    & 93.4  & 116.7 & 109.1 & 99.2  & 103.5 & 124.7 & 93.1  & 110.2 & 102.6 & 100.9 & 109.1 & 53.3    \\
5934.65       & 26         & 3.93  & -1.02    & 103   & 113.2 & 105.3 & 106.6 & 107.1 & 110.4 & 94.7  & 109.2 & 98.1  & 101.7 & 107.3 & 75      \\
6024.05       & 26         & 4.55  & -0.06    & 122.5 & 129.6 & 132.7 & 126.6 & 139   & 131.3 & 133.5 & 138   & 132   & 129.4 & 136.6 & 110.4   \\
6027.05       & 26         & 4.08  & -1.09    & 92.1  & 100.3 & 92.4  & 98.5  & 89.5  & 96.3  & 89.7  & 93.9  & 89.5  & 93.7  & 99.3  & 62.5    \\
6056          & 26         & 4.73  & -0.4     & 89.3  & 99.1  & 92.3  & 97.8  & 95.6  & 99.5  & 83.9  & 94.4  & 88.2  & 93.6  & 94.3  & 71.1    \\
6079          & 26         & 4.65  & -0.97    & 65.1  & 72.5  & 75.2  & 70.2  & 64.8  & 76.4  & 62.1  & 73    & 67    & 66.2  & 75    & 47.4    \\
6093.64       & 26         & 4.61  & -1.35    & 52.5  & 58.7  & 54.7  & 51    & 54.8  & 58.3  & 44    & 56.2  & 48.3  & 56.1  & 52.2  & 30.1    \\
6096.66       & 26         & 3.98  & -1.78    & 65    & 68.5  & 66    & 68.1  & 64.7  & 69.3  & 53.9  & 71.4  & 60.6  & 63.7  & 67.9  & 37.2    \\
6120.24       & 26         & 0.91  & -5.95    & 33.7  & 39.4  & 41.4  & 31.4  & 30.9  & 48.9  & 15.6  & 38.1  & 30.6  & 32.4  & 41.7  & 5.1     \\
6151.61       & 26         & 2.18  & -3.29    & 94.3  & 100.6 & 93.2  & 96.5  & 93.9  & 106.6 & 84.2  & 99.3  & 92.4  & 93.8  & 101.1 & 49.2    \\
6157.72       & 26         & 4.08  & -1.11    & 99.6  & 110.3 & 100.8 & 93.8  & 102.1 & 112.1 & 91.1  & 105.2 & 92.7  & 97.7  & 106.6 & 63.5    \\
6165.36       & 26         & 4.14  & -1.47    & 72.1  & 78.7  & 77.9  & 78.7  & 75.4  & 83.5  & 68    & 78.7  & 69.6  & 75    & 80.5  & 44      \\
6173.33       & 26         & 2.22  & -2.88    & 109.1 & 124.4 & 124.3 & 117.2 & 115.3 & 132.3 & 109.4 & 123.1 & 111.9 & 114.8 & 123.9 & 67.7    \\
6187.99       & 26         & 3.94  & -1.57    & 83.4  & 84.9  & 78.1  & 76.4  & 77.2  & 89.3  & 75    & 83.4  & 74.3  & 75.6  & 83.6  & 47.7    \\
6200.31       & 26         & 2.61  & -2.44    & 115.4 & 126.6 & 122.3 & 121.7 & 115.5 & 128.1 & 117.4 & 121.1 & 112.2 & 112.3 & 121.8 & 71.7    \\
6322.68       & 26         & 2.59  & -2.43    & 116.2 & 125.4 & 119.8 & 115.1 & 116.2 & 131.6 & 114.5 & 126   & 116.7 & 120.1 & 128.6 & 78.6    \\
6380.74       & 26         & 4.19  & -1.32    & 88.2  & 92.6  & 91.2  &  ---  & 94.2  & 103.6 & 90.8  & 97.7  & 83.4  & 84.6  &  ---  & 53.8    \\
6392.53       & 26         & 2.28  & -4.03    & 55.9  & ---   & 61.6  & 64.2  & 50.6  & 65.1  & ---   & 54.9  &  ---  & 59.6  & 65.4  & 18.2    \\
6419.95       & 26         & 4.73  & -0.09    & 102.7 & ---   & 121.5 & ---   & 119.4 & 121.8 & 125.9 & 128.7 & 111.5 & 111.8 & 128.1 & 87      \\
6436.4        & 26         & 4.19  & -2.46    & 33.8  & 41.6  & 38.3  & 33.3  & 31.7  & 39.1  & 26.4  & 36.7  & 27.9  & 30.2  & 34.6  & 11.1    \\
6469.19       & 26         & 4.84  & -0.62    & 89.4  & 102   & 93.2  & 87.3  & 92.4  & 103.1 & 80.7  & 98.3  & 85.7  & 91.4  &  ---  & 58.4    \\
6518.36       & 26         & 2.83  & -2.3     & 91.6  & 102.1 & 99.7  & 94.4  & ---   & 117.5 & 86.8  & 104.8 & 96.1  & 97.4  & 107.4 & 58.1    \\
6574.22       & 26         & 0.99  & -5.02    & 82.8  & 96.7  & 89.5  & 90.3  & 86.5  & 109.6 & 69.7  & 92.5  & 84.8  & 86.3  & 94.1  & 29      \\
6591.31       & 26         & 4.59  & -2.07    & 30.3  & 31.3  & 30.4  & ---   & 25.7  & 30.3  & ---   & 33.6  & 24.3  & 27.8  & 36.1  & 10.5    \\
6593.87       & 26         & 2.44  & -2.42    & 139.1 & 148.3 & 136.9 & 142.8 & 134.9 & 148.9 & 130.2 & 146   & 131.3 & 135.6 & 144   & 87.5    \\
6597.56       & 26         & 4.8   & -0.92    & 60.5  & 65.1  & 67.5  & 72.5  & 65.6  & 72.1  & ---   & 63.3  & 61    & 65.5  & 66    & 42.4    \\
6608.02       & 26         & 2.28  & -4.03    & 52.7  & 64    & 53.7  & 61.3  & 61.9  & 72.4  & 47.2  & 62.5  & 56.1  & 53.1  & 64.4  & 17.1    \\
6609.11       & 26         & 2.56  & -2.69    & 112.8 & 125.4 & 114.1 & 117.3 & 121.6 & 137.8 & 110.5 & 124.2 & 112.6 & 113   & 125.1 & 68.2    \\
6703.56       & 26         & 2.76  & -3.16    & 77.5  & 88.2  & 84.5  & 91.2  & 81.2  & 98.9  & 74.6  & 90.3  & 74.9  & 78.9  & 86.4  & 37.8    \\
6704.48       & 26         & 4.22  & -2.66    & 16.2  & 20.3  & 23.1  & 21.2  & 20.5  & 19.9  & 14.2  & 20    & 18.8  & 14.9  & 17.4  & 6.1     \\
6710.31       & 26         & 1.8   & -4.88    & 62.3  & 80.3  & 72.6  & 68.5  & 69.5  & 90.6  & 56.8  & 76.3  & 61    & 67.9  & 76.1  & 15.7    \\
6713.74       & 26         & 4.79  & -1.6     & 42.8  & 42    & 39.6  & 43.9  & 40.7  & 45.8  & 30    & 42.2  & 35.6  & 35.8  & 42.3  & 21.4    \\
6739.52       & 26         & 1.56  & -4.95    & 44.4  & 49.1  & 43.6  & 49.9  & ---   & 66.3  & 37    & 51    & ---   & 44.6  & 53.1  & 11.8    \\
6750.15       & 26         & 2.42  & -2.62    & 120   & 129.4 & 127.5 & 122.4 & 119.9 & 139.1 & 111.5 & 125.1 & 117.8 & 119.6 & 130.2 & 76.2    \\
6752.7        & 26         & 4.64  & -1.2     & 60.2  & 77.2  &  ---  & 69.4  & 71.4  & 80.3  & ---   & 80.4  & 64.9  & 71.9  & 74    & 38.2    \\
6793.25       & 26         & 4.07  & -2.47    & 27.4  &  ---  &  ---  & 28.9  &  ---  &  ---  & 22.2  &  ---  &  ---  &  ---  & 32.7  & 13.2    \\
6806.84       & 26         & 2.73  & -3.21    & 76    & 85.2  & 76.4  & 74.4  & 77.9  & 93.3  & 71.4  & 83.7  & 72.2  & 76.1  & 87.1  & 34      \\
6810.26       & 26         & 4.61  & -0.99    & 72.6  & 75.2  & 72.9  & 73.4  & 69.1  & 79.9  & 70.6  & 80.5  & 68.3  & 72.5  & 76.2  & 50      \\
6820.37       & 26         & 4.64  & -1.17    & 65.6  & 73.2  & 73    & 75.1  & 68.1  & 75.9  & 60.8  & 71.6  & 61.8  & 64.6  & 71.9  & 40.9    \\
6858.15       & 26         & 4.61  & -0.93    & 73.6  & 80    & 82.9  & 80.6  & 77.2  & 86.1  & 72.5  & 80.2  & 72.5  & 78.7  & 81    & 50.2    \\
6551.67       & 26         & 0.99  & -5.79    & ---   & 51.6  & 46.3  & 45.5  & 36.4  & 63.4  &  ---  & 53    & 41.1  &  ---  & 51.9  & 6.1     \\
6646.93       & 26         & 2.61  & -3.99    & ---   & 50.4  & 44.4  & 42.4  & 41.8  & 60.1  &  ---  & 47.6  & 36.3  & 37.7  & ---   & 8.2     \\
6653.85       & 26         & 4.14  & -2.52    & ---   & 27.5  & 22.6  & 28.4  & 26.3  & 30.4  & 22    & 27.2  & 24.2  & 23.6  & 27.1  & 10.9    \\
6699.14       & 26         & 4.59  & -2.19    & ---   & 30.4  & 24    & 23.9  & 20.3  & 30.1  & 12.4  & 22.9  & 19.9  & ---   & 24.8  & 7.5     \\
6745.95       & 26         & 4.07  & -2.77    & ---   & 19    & ---   &  ---  & ---   &  ---  & ---   & ---   &  ---  & ---   & 21.1  & 8.3     \\
6851.63       & 26         & 1.61  & -5.32    & ---   & 47    & 41.6  & 42    & 35    & 54.2  & 21.5  & 39.8  & 35.2  & 42.1  & 37.6  & 6.7     \\
7132.98       & 26         & 4.08  & -1.61    & ---   & 72    & 76.6  & ---   & ---   &  ---  & ---   & ---   & ---   & ---   & ---   & 42.5    \\
6170.5        & 26         & 4.8   & -0.38    & ---   &  ---  & 117.5 & ---   & ---   &  ---  & 115   & ---   & ---   & 113.2 & ---   & 82.9    \\
6783.7        & 26         & 2.59  & -3.98    & ---   &  ---  &  ---  & ---   & ---   & 70.3  & ---   & 63.3  & 50.8  & 52.3  & 64.7  & 14.3    \\
4993.34       & 26.1       & 2.81  & -3.67    & 59.6  &  ---  & 68.4  & 56.9  & 52.9  & 62.6  & ---   & 63.1  & 60.6  & ---   & 63.2  & 38      \\
5132.65       & 26.1       & 2.81  & -4       & 42.1  & 55.5  & 49.5  & 41.7  & 44.7  & ---    & 37.7  & 44.4  & 45.1  & 43.6  & 43.9  & 23.8    \\
5197.55       & 26.1       & 3.23  & -2.25    & 107.4 & 110.6 & 106.9 &  ---  & ---   & 110.1 & 115   & 111.1 & 102   & 108.5 &       & 81.9    \\
5234.61       & 26.1       & 3.22  & -2.24    & 111.8 &       & 104   & 105.3 & 102.7 & 101.4 & ---   & 110.7 & 102.5 & 103.8 & 103.8 & 81.9    \\
5284.09       & 26.1       & 2.89  & -3.01    & 86.6  & 95.7  &  ---  &  ---  & 87.5  & ---   & ---   & ---   &  ---  & ---   &  ---  & 66.7    \\
5325.55       & 26.1       & 3.22  & -3.17    & 62    & 56.9  & 60.7  & 62.5  & 58    & 58.5  & ---   & 60.9  & 60.8  & ---   & 60.2  & 38.7    \\
5414.04       & 26.1       & 3.22  & -3.62    & 42.2  & 46.9  & 50.4  & 44.1  & 43.2  & ---   & 43.1  & ---   & 43.9  & ---   & 45.5  & 25.9    \\
5425.24       & 26.1       & 3.2   & -3.21    & 67.9  & 66.4  & 60.9  & 64.8  & 59.1  & 59.4  & 69.1  & 60.3  & 58.5  & 63.2  & 61.6  & 39.6    \\
5991.36       & 26.1       & 3.15  & -3.56    & 52.3  & 56.3  & ---   & 52.5  & 52.1  & 53.6  & ---   & 60    & 51.2  & 53.6  & 54.4  & 29.9    \\
6084.09       & 26.1       & 3.2   & -3.8     & 40.3  & 47.8  & 44.4  & ---   &  ---  & 45.2  & ---   & 46.7  & 40.5  & 42.6  & 42.6  & 22.2    \\
6149.24       & 26.1       & 3.89  & -2.72    & 51.5  & 54.3  & 56.5  & 53    & 46.7  & 48.4  & 55.6  & ---   & 52.8  & 53.2  & 57.6  & 37.7    \\
6247.54       & 26.1       & 3.89  & -2.34    & 70.6  & 74.8  & 73.8  & 72.8  & 68.6  & 65.8  & 76.8  & 74.4  & 70.4  & 79.2  & 75.2  & 55.9    \\
6416.92       & 26.1       & 3.89  & -2.68    & 55.2  & 61.2  & 56.6  & 58.7  & 55.3  & 60.6  & 61.4  & 57.4  & 55.1  & 56.8  & 59.7  & 39.6    \\
6432.68       & 26.1       & 2.89  & -3.58    & 61.8  & 64.2  & 66.6  & 63.9  & 57.9  & 61.6  & 64.3  & 63.4  & 66.2  & 65.8  & 63.2  & 43.1    \\
4607.34       & 38         & 0     & 0.283    & 88.7  & 91.4  & 89.7  & 82.6  & 93    & 98.1  & 93.1  & 91.2  & 84.7  & 88    & 94.1  & 41      \\
4883.68       & 39.1       & 1.08  & 0.07     & 91.1  & ---   &  ---  & ---   &  ---  & ---   & ---   & ---   &  ---  & ---   & ---   & 60.1    \\
5087.43       & 39.1       & 1.08  & -0.17    & 81.7  & 88.5  & 81.6  & 81.6  & 88.7  & 92.1  & 95.9  & 91.7  & 85.9  & 87.8  & 87.8  & 48.8    \\
5200.42       & 39.1       & 0.99  & -0.57    & 73.2  & 85.1  & 77.9  & 75.6  & 88.2  & 92.3  & ---   & 87.5  & 80.8  & 81.7  & 84.6  & 38.9    \\
5205.72       & 39.1       & 1.03  & -0.34    & 75.7  & ---   & ---   &  ---  &  ---  & ---   & ---   &  ---  & ---    & ---  & ---   & 41.4    \\
5289.82       & 39.1       & 1.03  & -1.85    & 20.4  & 26.1  & ---   & 23.3  & 30    & 30.1  & 28.3  & 28.6  & 25.1  & 26.7  & 25.7  & 5.2     \\
5402.78       & 39.1       & 1.84  & -0.44    & ---   & 46.6  & 40.4  & 42.8  & 43.5  & 49.1  & 43.1  & 46.1  & 39.8  & 40.1  & 44.5  & 13      \\
5385.13       & 40         & 0.52  & -0.64    & 14.3  & 21    & 17.1  & ---   & 13.3  & 26.9  & ---   & 19.7  & ---   & 15    & 17.4  & 1.8     \\
6127.46       & 40         & 0.15  & -1.06    & 26.5  & 26    & 22.9  & 20.1  & 24.1  &  ---  & 22.8  & 27.9  & 25.2  & 24.4  & 29.1  & 3.8     \\
6134.57       & 40         & 0     & -1.28    & 17.4  & 26.7  & 28.2  & 18.4  & 19.5  & 31.6  & 12.9  & 26.1  & 19.9  & 23.8  & 24.4  & 2.2     \\
6143.18       & 40         & 0.07  & -1.1     & 28.4  & 33.3  & 27.2  & 21.6  & 22.9  & ---   &  ---  & 30.2  & 23.8  & 17.7  & 29.1  & 3       \\
5303.53       & 57.1       & 0.32  & -1.35    & 25.1  & 31.9  & 22.4  & 18.2  & 28.5  & 34.2  & 23.7  & 31.5  & 27.3  & 25.9  & 35.7  & 3.6     \\
6390.48       & 57.1       & 0.32  & -1.41    & 22.9  & 28.2  & 32.2  & 26.2  & 29    & 42.2  & 24.2  & 33.1  & 33.9  & 32    & 34    & 3.9     \\
5880.63       & 57.1       & 0.24  & -1.83    & ---   & 20.2  & ---   & 11    & ---   & ---   &  ---  & ---   & 17    & ---   & ---   & 1.4     \\
4628.16       & 58.1       & 0.52  & -0.74    & 57.6  & 66.4  & 69.7  & 62    & 63.5  & ---   & 63.1  & 67.9  & 55.9  & 67.4  & 71.5  & 17.7    \\
5187.46       & 58.1       & 1.21  & 0.3      & 29    & 31.2  & 36.7  & 36.4  & 31.9  & 42.1  & ---   & 37.3  & 29.5  & 31.4  & 30.1  & 7.5     \\
5274.24       & 58.1       & 1.28  & 0.389    & 34    & 43.8  & 40.4  & 35.7  & 44.1  & 47.4  & 35.1  & 43.2  & 39.4  & 40.3  & 47.8  & 9.8     \\
5472.3        & 58.1       & 1.25  & -0.19    & 13.5  & 19.1  & 18.4  & ---   & ---   & 23.9  & 14    & 21.2  & ---   & 17.3  & 18.8  & 2.4     \\
4811.34       & 60.1       & 0.06  & -1.015   & 43.9  & 65.2  & 48.2  & 57.6  & 53.8  & 72.7  & 37    & 66.5  & 55.2  & 57.9  & 59.9  & 9.3     \\
4959.12       & 60.1       & 0.06  & -0.916   & 70.5  & 90.1  & 84.6  & 75.7  & 75.1  & 96.1  & ---   & 85.3  & 75.5  & 76.5  & 80.3  & 32.4    \\
5130.59       & 60.1       & 1.3   & 0.1      & 38.9  & ---   & ---   & ---   & ---   & ---   & ---   & ---   & ---   & ---   & 44.9  & 12.6    \\
5319.81       & 60.1       & 0.55  & -0.35    & 50.6  & 67    & 61    & 61    & ---   & ---   & ---   & 61.4  & 60.1  & 54.3  & 64.1  & 13      \\
5740.88       & 60.1       & 1.16  & -0.56    & 12.7  & ---   & 19.8  & ---   & 15    & 23.6  & ---   & 19.8  & ---   &  ---  & 17.2  & 2.4     \\
5234.19       & 60.1       & 0.55  & -0.46    &  ---  & 57.8  & 40.6  & ---   & 31.2  & ---   & 32.9  & 57.1  & ---   &  ---  & ---   & 5.6     \\
5311.46$^{7}$   & 60.1   & 0.98  & -0.56    &  ---  &  ---  &  ---  & ---   & ---   & ---   & ---   & ---   & ---   & 18.8  & ---   & 2.3     \\
\hline
\hline
\end{longtable}

\normalsize
